Towards Robust Probabilistic Modeling on SO(3) via Rotation Laplace Distribution

Estimating the 3DoF rotation from a single RGB image is an important yet challenging problem. As a popular approach, probabilistic rotation modeling additionally carries prediction uncertainty information, compared to single-prediction rotation regression. For modeling probabilistic distribution over SO(3), it is natural to use Gaussian-like Bingham distribution and matrix Fisher, however they are shown to be sensitive to outlier predictions, e.g. $180^\circ$ error and thus are unlikely to converge with optimal performance. In this paper, we draw inspiration from multivariate Laplace distribution and propose a novel rotation Laplace distribution on SO(3). Our rotation Laplace distribution is robust to the disturbance of outliers and enforces much gradient to the low-error region that it can improve. In addition, we show that our method also exhibits robustness to small noises and thus tolerates imperfect annotations. With this benefit, we demonstrate its advantages in semi-supervised rotation regression, where the pseudo labels are noisy. To further capture the multi-modal rotation solution space for symmetric objects, we extend our distribution to rotation Laplace mixture model and demonstrate its effectiveness. Our extensive experiments show that our proposed distribution and the mixture model achieve state-of-the-art performance in all the rotation regression experiments over both probabilistic and non-probabilistic baselines.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> response_tex/fig_vis_distribution.tex <==
\begin{figure*}[t]
    \centering
    % \vspace{-6mm}
    % \hspace{-3mm}
    \begin{tabular}{ccc}
    \includegraphics[clip,trim=1cm 3cm 1cm 0cm,width=0.18\linewidth]{figures/vis_distribution/Lap_Id_5_5_5.png}
    &\includegraphics[clip,trim=1cm 3cm 1cm 0cm,width=0.18\linewidth]{figures/vis_distribution/Lap_Id_25_25_25.png}
    &\includegraphics[clip,trim=1cm 3cm 1cm 0cm,width=0.18\linewidth]{figures/vis_distribution/Lap_Id_25_5_1.png}
    \\
    \small{(a) diag(5, 5, 5)} &\small{(b) diag(25, 25, 25)} &\small{(c) diag(25, 5, 1)} 
    \\
    \includegraphics[clip,trim=1cm 3cm 1cm 0cm,width=0.18\linewidth]{figures/vis_distribution/Lap_Tx_25_5_1.png}
    &\includegraphics[clip,trim=1cm 3cm 1cm 0cm,width=0.18\linewidth]{figures/vis_distribution/Lap_Ty_25_5_1.png}
    &\includegraphics[clip,trim=1cm 3cm 1cm 0cm,width=0.18\linewidth]{figures/vis_distribution/Lap_Tz_25_5_1.png}
    \\
    \small{(d) $\mathbf{T}_x$ diag(25, 5, 1) $\mathbf{T}_x^T$} &\small{(e) $\mathbf{T}_y$ diag(25, 5, 1) $\mathbf{T}_y^T$} &\small{(f) $\mathbf{T}_z$ diag(25, 5, 1) $\mathbf{T}_z^T$} 
    
    \end{tabular}
    \vspace{-2mm}
    \caption{\small \textbf{Effect of the parameter $\mathbf{A}$ on the shape of rotation Laplace distribution.} $\mathbf{T}_i$ refers to the rotation matrix by rotating $\pi/4$ around $e_i$.}
    \vspace{-2mm}
	\label{fig:vis_shape}
\end{figure*}

==> response_tex/math_constant.tex <==
% \todo{we have verified the equations by sampling?}
Many thanks for the advice. We firstly show that the normalization factor depends only on $\mathbf{S}$.
\begin{proof}
\begin{equation}
\footnotesize
\begin{aligned}
    F(\mathbf{A}) 
    &= \int_{\SO} \frac{\exp\left(-\sqrt{\operatorname{tr}\left(\mathbf{S} - \mathbf{A}^T \mathbf{R}\right)}\right)}
    {\sqrt{\operatorname{tr}\left(\mathbf{S} -\mathbf{A}^T \mathbf{R}\right)}} \mathrm{d}\mathbf{R}\\ 
    & = \int_{\SO} \frac{\exp\left(-\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{U}^T\mathbf{R}\mathbf{V})}\right)}{\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{U}^T\mathbf{R}\mathbf{V})}} \mathrm{d}\mathbf{R} \\
    & \xlongequal{\mathbf{R}'=\mathbf{U}^T\mathbf{R}\mathbf{V}}  \int_{\SO} \frac{\exp\left(-\sqrt{\operatorname{tr}\left(\mathbf{S} - \mathbf{S}\mathbf{R}'\right)}\right)}
    {\sqrt{\operatorname{tr}\left(\mathbf{S} -\mathbf{S}\mathbf{R}'\right)}} \mathrm{d}\mathbf{R}'\
\end{aligned}
\end{equation}
\end{proof}

We then try to derive expression of the normalization factor. We have verified our solutions by comparing with numerical results via discretization.

Denote $s_1, s_2, s_3$ as the singular values of $\mathbf{A}$.
Considering the transformation between rotation matrix and unit quaternion
    \begin{equation}
    \footnotesize
        \mathbf{R}' = \gamma(\mathbf{q}) = \begin{pmatrix} 1-2y^2-2z^2 & 2xy-2zw & 2xz+2yw \\ 2xy+2zw & 1-2x^2-2z^2 & 2yz-2xw \\ 2xz-2yw & 2yz+2xw & 1-2x^2-2y^2 \end{pmatrix},
    \label{eq:r_to_q}
    \end{equation}
we define 
% $t_1=2(s_2+s_3)$, $t_2=2(s_3+s_1)$, $t_3=2(s_1+s_2)$ and $k=t_1x_0^2+t_2y_0^2+t_3z_0^2$
\begin{equation}
    \footnotesize
    \begin{aligned}
        t_1&=2(s_2+s_3) \\
        t_2&=2(s_1+s_3) \\
        t_3&=2(s_1+s_2) \\
        %k&=t_1x_0^2+t_2y_0^2+t_3z_0^2 \\
    \end{aligned}
    \label{eq:t123}
\end{equation}
the normalizing factor can be expressed as a one-dimensional integration:
    \begin{equation}
    \footnotesize
        F(\mathbf{A})=\frac{2}{\pi}\left(\int_{t_1}^{t_2}\frac{\left(\mathbf{L}_{-1}(\sqrt{k})-\mathbf{I}_{1}(\sqrt{k})\right)\mathbf{K}\left(\frac{(k-t_1)(t_3-t_2)}{(t_1-t_2)(k-t_3)}\right)}{\sqrt{k(t_2-t_1)(t_3-k)}}\mathrm{d}k
        + \int_{t_2}^{t_3}\frac{\left(\mathbf{L}_{-1}(\sqrt{k})-\mathbf{I}_{1}(\sqrt{k})\right)\mathbf{K}\left(\frac{(k-t_3)(t_1-t_2)}{(t_3-t_2)(k-t_1)}\right)}{\sqrt{k(t_2-t_3)(t_1-k)}}\mathrm{d}k\right)
    \end{equation}
where $\mathbf{L}$ is the modified Struve function, $\mathbf{I}$ is the modified Bessel function of the first kind, and $\mathbf{K}$ is the complete elliptic integral of the first kind.

Specifically, when $s_1 = s_2 = s_3 = s$, it can be simplified as 
\begin{equation}
\footnotesize
    F(\mathbf{A})=\frac{\mathbf{L}_{-1}(2\sqrt{s})-\mathbf{I}_1(2\sqrt{s})}{\sqrt{s}}
\end{equation}
%where $_0\tilde{\mathbf{F}}_1$ is regularized confluent hypergeometric function.

\begin{proof}
    Given $\mathbf{R}'=\mathbf{U}^T\mathbf{R}\mathbf{V}$, and considering Eq. \ref{eq:r_to_q}
    we have
    \begin{equation}
    \footnotesize
        \operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{R}')=2(s_2+s_3)x^2+2(s_1+s_3)y^2+2(s_1+s_2)z^2
    \end{equation}
    Define $\theta$ as the rotation angle, and then the quaternion $(w,x,y,z)$ can be expressed as 
    \begin{equation}
        \footnotesize
        (w,x,y,z) = (\cos\theta, \sin\theta x_0, \sin\theta y_0, \sin\theta z_0)
    \end{equation}
    satisfying $x_0^2+y_0^2+z_0^2=1$. Thus we can first integrate over $\theta$, then integrate over $a=(x_0, y_0, z_0)\in\mathcal{S}^2$.
    Considering Eq. \ref{eq:t123}, we have
    \begin{equation}
    \footnotesize
    \begin{aligned}
        F(\mathbf{A})&=\frac{1}{2\pi^2}\int_{\SO} \frac{\exp\left(-\sqrt{2(s_2+s_3)x^2+2(s_1+s_3)y^2+2(s_1+s_2)z^2}\right)}{\sqrt{2(s_2+s_3)x^2+2(s_1+s_3)y^2+2(s_1+s_2)z^2}} \\
        &=\frac{1}{2\pi^2}\int_{\SO}\frac{\exp\left(-\sin{\theta}\sqrt{2(s_2+s_3)x_0^2+2(s_1+s_3)y_0^2+2(s_1+s_2)z_0^2}\right)}{\sin{\theta}\sqrt{2(s_2+s_3)x_0^2+2(s_1+s_3)y_0^2+2(s_1+s_2)z_0^2}} \\
    \end{aligned}
    \end{equation}

    By defining 

    \begin{equation}
    \footnotesize
        k=t_1x_0^2+t_2y_0^2+t_3z_0^2
    \end{equation}

    we have
    
    \begin{equation}
    \footnotesize
    \begin{aligned}
        F(\mathbf{A})&=\frac{1}{2\pi^2}\int_{\SO}\frac{\exp\left(-\sqrt{k}\sin{\theta}\right)}{\sqrt{k}\sin{\theta}} \\
        &=\frac{1}{2\pi^2}\int_{\mathcal{S}^2} \frac{1}{\sqrt{k}} \int_{0}^{\pi} \sin{\theta}\exp\left(-\sqrt{k}\sin{\theta}\right) \mathrm{d}\theta \mathrm{d}a \\
        &=\frac{1}{2\pi}\int_{\mathcal{S}^2} \frac{\mathbf{L}_{-1}(\sqrt{k})-\mathbf{I}_{1}(\sqrt{k})}{\sqrt{k}} \mathrm{d}a \\
        &=\frac{1}{2\pi}\left(\int_{t_1}^{t_2}S_1(k)\frac{\mathbf{L}_{-1}(\sqrt{k})-\mathbf{I}_{1}(\sqrt{k})}{\sqrt{k}}\mathrm{d}k+\int_{t_2}^{t_3}S_2(k)\frac{\mathbf{L}_{-1}(\sqrt{k})-\mathbf{I}_{1}(\sqrt{k})}{\sqrt{k}}\mathrm{d}k\right)
    \end{aligned}
    \label{eq:f_to_s}
    \end{equation}
where $S_1(k)$  is computed as 
    \begin{equation}
    \footnotesize
    \begin{aligned}
        S_1(k)&=\int_0^{\sqrt{\frac{k-t_1}{t_2-t_1}}}\frac{4}{(t_3-t_1)xz}\mathrm{d}y \\
        &= \int_0^{\sqrt{\frac{k-t_1}{t_2-t_1}}}\frac{4}{\sqrt{k-t_1+t_1y^2-t_2y^2}\sqrt{-k+t_3-t_3y^2+t_2y^2}}\mathrm{d}y \\
        &=  \frac{4\mathbf{K}(\frac{(k-t_1)(t_3-t_2)}{(t_1-t_2)(k-t_3)})}{\sqrt{(t_2-t_1)(t_3-k)}} 
    \end{aligned}
    \label{eq:s1}
    \end{equation}
    Similarily, we have 
    \begin{equation}
    \footnotesize
    \begin{aligned}
        S_2(k)&=\frac{4\mathbf{K}(\frac{(k-t_3)(t_1-t_2)}{(t_3-t_2)(k-t_1)})}{\sqrt{(t_2-t_3)(t_1-k)}}
    \end{aligned}
    \label{eq:s2}
    \end{equation}
    Combining Eq. \ref{eq:f_to_s}, Eq. \ref{eq:s1}, and \ref{eq:s2} together, we have
    \begin{equation}
    \footnotesize
        F(\mathbf{A})=\frac{2}{\pi}\left(\int_{t_1}^{t_2}\frac{\left(\mathbf{L}_{-1}(\sqrt{k})-\mathbf{I}_{1}(\sqrt{k})\right)\mathbf{K}\left(\frac{(k-t_1)(t_3-t_2)}{(t_1-t_2)(k-t_3)}\right)}{\sqrt{k(t_2-t_1)(t_3-k)}}\mathrm{d}k
        + \int_{t_2}^{t_3}\frac{\left(\mathbf{L}_{-1}(\sqrt{k})-\mathbf{I}_{1}(\sqrt{k})\right)\mathbf{K}\left(\frac{(k-t_3)(t_1-t_2)}{(t_3-t_2)(k-t_1)}\right)}{\sqrt{k(t_2-t_3)(t_1-k)}}\mathrm{d}k\right)
    \end{equation}
    
Specifically, when $s_1=s_2=s_3=s$, 
\begin{equation}
    \footnotesize
    \begin{aligned}
        t_1&=2(s_2+s_3)=4s \\
        t_2&=2(s_1+s_3)=4s \\
        t_3&=2(s_1+s_2)=4s \\
        k&=t_1x_0^2+t_2y_0^2+t_3z_0^2=4s(x_0^2+y_0^2+z_0^2)=4s \\
    \end{aligned}
\end{equation}
    Thus with Eq. \ref{eq:f_to_s} we have,
    \begin{equation}
    \footnotesize
    \begin{aligned}
        F(\mathbf{A})&=\frac{1}{2\pi}\int_{\mathcal{S}^2} \frac{\mathbf{L}_{-1}(\sqrt{k})-\mathbf{I}_{1}(\sqrt{k})}{\sqrt{k}} \mathrm{d}a \\
        &=\frac{1}{4\pi}\int_{\mathcal{S}^2} \frac{\mathbf{L}_{-1}(2\sqrt{s})-\mathbf{I}_{1}(2\sqrt{s})}{\sqrt{s}} \mathrm{d}a \\
        &=\frac{\mathbf{L}_{-1}(2\sqrt{s})-\mathbf{I}_1(2\sqrt{s})}{\sqrt{s}}
    \end{aligned}
    \end{equation}
\end{proof}

\jiangran{We provide the analytical expression of the normalization factor in Section 4.6 of the revised manuscript.}

==> response_tex/math_mean.tex <==
\textbf{Chordal Mean.} We define the \textit{chordal mean} \cite{hartley2013rotation,sarlette2009consensus,moakher2002means} of the distribution under the chordal metrics over $\SO$:
% . Given N rotations sampled from rotation Laplace distribution, the \textit{mean} of the distribution is defined as
\begin{equation}
% \footnotesize
    \Bar{\mathbf{R}} = \argmin_{\mathbf{R}\in \SO} \int_{\mathbf{R}^* \in \SO} p(\mathbf{R}^*) d_{\text{chord}}(\mathbf{R}, \mathbf{R}^*) \mathrm{d}\mathbf{R}^*
    % \| \mathbf{R} - \mathbf{R}^* \|^2
    \label{eq:definition}
\end{equation}
where $d_{\text{chord}}(\cdot, \cdot)$ denotes the L2 chordal metrics of two rotations:
\begin{equation}
    d_{\text{chord}}(\mathbf{R}_1, \mathbf{R}_2) = \| \mathbf{R}_1 - \mathbf{R}_2 \|_F^2
    % \arccos\left( \frac{\tr{\mathbf{R}_1^T\mathbf{R}_2}-1}{2} \right)
\end{equation}


The mean of our distribution under the chordal metrics is:
\begin{equation}
% \footnotesize
    \Bar{\mathbf{R}} = \mathbf{UV}^T
\end{equation}


% \begin{preliminary}
%     \begin{equation}
%         d_g(\mathbf{R}_1, \mathbf{R}_2) \propto \|\mathbf{R}_1 - \mathbf{R}_2\|
%     \end{equation}
%     \label{pre:distance}
% \end{preliminary}

% \begin{proof}
%     \todo{}
% \end{proof}





% The mean of our distribution under the chordal metrics is:
% \begin{equation}
% % \footnotesize
%     \Bar{\mathbf{R}} = \mathbf{UV}^T
% \end{equation}

\begin{proof}
    % Considering Eq. \ref{eq:definition} and Preliminary \ref{pre:distance},
    \begin{equation}
    \footnotesize
    \begin{aligned}
        % \Bar{\mathbf{R}} &= \argmin_{\mathbf{R}\in \SO} \int_{\mathbf{R}^* \in \SO} p(\mathbf{R}^*) d_g(\mathbf{R}, \mathbf{R}^*) \mathrm{d}\mathbf{R}^* \\
        \Bar{\mathbf{R}}&= \argmin_{\mathbf{R}\in \SO} \int_{\mathbf{R}^* \in \SO} p(\mathbf{R}^*) \| \mathbf{R} - \mathbf{R}^* \|^2_F \mathrm{d}\mathbf{R}^*
    \end{aligned}
    \end{equation}
    With Preliminary \ref{pre:norm},
    \begin{equation}
    \footnotesize
    \begin{aligned}
        \Bar{\mathbf{R}} 
        &= \argmin_{\mathbf{R}\in\SO} \left(-\int_{\mathbf{R}^* \in \SO} p(\mathbf{R}^*) \gamma^{-1}(\mathbf{R} )^T \gamma^{-1}(\mathbf{R}^*) \gamma^{-1}(\mathbf{R}^*)^T \gamma^{-1}(\mathbf{R}) \mathrm{d}\mathbf{R}^* \right) \\
        &= \argmin_{\mathbf{R}\in\SO} \left( -\gamma^{-1}(\mathbf{R})^T
        \left( \int_{\mathbf{R}^*\in\SO} p(\mathbf{R}^*) \gamma^{-1}(\mathbf{R}^*) \gamma^{-1}(\mathbf{R}^*) \mathrm{d}\mathbf{R}^* \right)  \gamma^{-1}(\mathbf{R})\right)
    \end{aligned}
    \end{equation}
    Let $\Bar{\mathbf{q}} = \gamma^{-1}(\Bar{\mathbf{R}})$, we have 
    \begin{equation}
    \footnotesize
        \Bar{\mathbf{q}} = \argmin_{\mathbf{q}\in \mathcal{S}^3}\left( -{\mathbf{q}}^T \left( \int_{\mathbf{q}^*\in \mathcal{S}^3} p(\mathbf{q}^*) \mathbf{q}^* \mathbf{q}^{*T} \mathrm{d}\mathbf{q}^*  \right) {\mathbf{q}} \right)
    \end{equation}
    We define
    \begin{equation}
    \footnotesize
    \footnotesize
        \mathcal{L}(\mathbf{q}) = -\mathbf{q}^{T} \left(
        \int_{\mathbf{q}^*\in \mathcal{S}^3} p(\mathbf{q}^*) \mathbf{q}^* \mathbf{q}^{*T} \mathrm{d}\mathbf{q}^*
        \right) \mathbf{q}
    \end{equation}
    then
    \begin{equation}
    \footnotesize
        \Bar{\mathbf{q}} = (\Bar{w}, \Bar{x}, \Bar{y}, \Bar{z}) = \argmin_{\mathbf{q}\in \mathcal{S}^3} \mathcal{L}(\mathbf{q})
    \end{equation}


    % We first consider the simple case when $\mathbf{A}=\mathbf{S}=\operatorname{diag}(s1, s2, s3)$. Otherwise, we apply a transformation $\mathbf{R}'=\mathbf{V}^T\mathbf{R}\mathbf{U}$.
    For rotation Laplace distribution,
    \begin{equation}
    \footnotesize
    \begin{aligned}
        p(\mathbf{R}; \mathbf{A}) 
        &= \frac{1}{F(\mathbf{A})} \frac{\exp\left(-\sqrt{\operatorname{tr}\left(\mathbf{S} - \mathbf{A}^T \mathbf{R}\right)}\right)}
        {\sqrt{\operatorname{tr}\left(\mathbf{S} -\mathbf{A}^T \mathbf{R}\right)}} \\ 
        & = \frac{1}{F(\mathbf{A})} \frac{\exp\left(-\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{U}^T\mathbf{R}\mathbf{V})}\right)}{\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{U}^T\mathbf{R}\mathbf{V})}} \\
        & \xlongequal{\mathbf{R}'=\mathbf{U}^T\mathbf{R}\mathbf{V}}  \frac{1}{F(\mathbf{A})} \frac{\exp\left(-\sqrt{\operatorname{tr}\left(\mathbf{S} - \mathbf{S}\mathbf{R}'\right)}\right)}
        {\sqrt{\operatorname{tr}\left(\mathbf{S} -\mathbf{S}\mathbf{R}'\right)}} 
    \end{aligned}
    \end{equation}

    
    Below we first consider the geodesic mean of  $\mathbf{R}'$, denoted as $\Bar{\mathbf{R}}'$, and then 
    \begin{equation}
        \Bar{\mathbf{R}} = \mathbf{U}\Bar{\mathbf{R}}'\mathbf{V}^T
        \label{eq:rprime}
    \end{equation}
    
    % We consider the simple case when $\mathbf{A}=\mathbf{S}$. Otherwise, we apply a transformation $\mathbf{R}'=\mathbf{V}^T\mathbf{R}\mathbf{U}$, such that the distribution follows the simple case.
    
    % Given $\mathbf{R}'=\mathbf{U}^T\mathbf{R}\mathbf{V}$, and c
    Considering the transformation between rotation matrix and unit quaternion Eq. \ref{eq:r_to_q},  we have 
    \begin{equation}
    \footnotesize
        p(w,x,y,z;\mathbf{A}) = \frac{1}{F(\mathbf{A})} \frac{\exp\left(
        -\sqrt{2(s_2+s_3) x^2 + 2(s_1+s_3) y^2 + 2(s_1+s_2)z^2}
        \right)}{\sqrt{2(s_2+s_3) x^2 + 2(s_1+s_3) y^2 + 2(s_1+s_2)z^2}}
        \label{eq:pdf_q}
    \end{equation}

    Given the even function property of Eq. \ref{eq:pdf_q}, we have
    \begin{equation}
    \footnotesize
        p(w,x,y,z) = p(w,-x,y,z) = p(w,x,-y,z) = p(w,x,y,-z)
    \end{equation}
    and 
    \begin{equation}
    \footnotesize
        \mathcal{L}(w,x,y,z) = \mathcal{L}(w,-x,y,z) = \mathcal{L}(w,x,-y,z) = \mathcal{L}(w,x,y,-z)
    \end{equation}
    and thus the four quaternions should all be the mean of the distibution: 
    $(\Bar{w}, \Bar{x}, \Bar{y}, \Bar{z})$, $(\Bar{w}, -\Bar{x}, \Bar{y}, \Bar{z})$, $(\Bar{w}, \Bar{x}, -\Bar{y}, \Bar{z})$, $(\Bar{w}, \Bar{x}, \Bar{y}, -\Bar{z})$.
    % $(w^*, -x^*, y^*, z^*)$, $(w^*, x^*, -y^*, z^*)$, $(w^*, x^*, y^*, -z^*)$
    Due to the uniqueness of the mean, the four quaternions should be identical, and thus $(\Bar{w}, \Bar{x}, \Bar{y}, \Bar{z})$ must be an item in the set $\mathcal{Q}=\{(1, 0, 0, 0)$, $(0, 1, 0, 0)$, $(0, 0, 1, 0)$, $(0, 0, 0, 1)\}$, i.e.,
    % one of the four values: $(1, 0, 0, 0)$, $(0, 1, 0, 0)$, $(0, 0, 1, 0)$, $(0, 0, 0, 1)$.
    % Since the mean of the distribution is unique, we denote it as $(w^*, x^*, y^*, z^*)$. 
    % Then $(w^*, -x^*, y^*, z^*)$, $(w^*, x^*, -y^*, z^*)$, $(w^*, x^*, y^*, -z^*)$ should be the same unit quaternion as $(w^*, x^*, y^*, z^*)$.
    % Therefore, $(w^*, x^*, y^*, z^*)$ must be one of the four values: $(1, 0, 0, 0)$, $(0, 1, 0, 0)$, $(0, 0, 1, 0)$, $(0, 0, 0, 1)$.
    \begin{equation}
    \footnotesize
        \Bar{\mathbf{q}} = (\Bar{w}, \Bar{x}, \Bar{y}, \Bar{z}) = \argmin_{\mathbf{q}\in \mathcal{Q}}
        \mathcal{L}(\mathbf{q})
    \end{equation}

    Now we compare $\mathcal{L}(1, 0, 0, 0)$, $\mathcal{L}(0, 1, 0, 0)$

    \begin{equation}
    \footnotesize
    \begin{aligned}
        \mathcal{L}(1, 0, 0, 0) 
        &= -(1, 0, 0, 0)\int_{\mathcal{S}^3}p(\mathbf{q}) \mathbf{q} \mathbf{q}^T \mathrm{d}\mathbf{q}
        \begin{pmatrix}
      1  \\
      0\\
      0 \\
      0
        \end{pmatrix}\\
        % &\xlongequal{\mathbf{q} = (w, x, y, z)}
        % &\overset{q = (w, x, y, z)}{=} 
        &=
        -\int_{\mathcal{S}^3}w^2  p(w,x,y,z) \mathrm{d}(w,x,y,z) \\
        &= -\frac{1}{2} \int_{\mathcal{S}^3} (w^2 p(w, x,y,z) + x^2 p(x, w,y,z) )
         \mathrm{d}(w, x, y,z) 
        \end{aligned}
        \end{equation}
    
    Similarly,
    \begin{equation}
    \footnotesize
    \begin{aligned}
         \mathcal{L}(0, 1, 0, 0) &=
         -\int_{\mathcal{S}^3}x^2  p(w,x,y,z) \mathrm{d}(w,x,y,z) \\
         &= -\frac{1}{2} \int_{\mathcal{S}^3} (x^2 p(w,x,y,z) +w^2 p(x,w,y,z)) 
         \mathrm{d}(w, x, y,z) 
    \end{aligned}
    \end{equation}

    
    Therefore,
    \begin{equation}
    \footnotesize
    \begin{aligned}
        &\mathcal{L}(0, 1, 0, 0) - \mathcal{L}(1, 0, 0, 0)  \\ &=
        \frac{1}{2} \int_{\mathcal{S}^3} ((w^2 p(w, x,y,z) + x^2 p(x, w,y,z) 
        - x^2 p(w,x,y,z) -w^2 p(x,w,y,z))
         \mathrm{d}(w, x, y,z) 
        \\ &= \frac{1}{2} \int_{\mathcal{S}^3}
        (w^2-x^2)(p(w,x,y,z) - p(x, w, y,z)) \mathrm{d}(w,x,y,z) 
    \end{aligned}
    \end{equation}

    
    Considering Eq. \ref{eq:pdf_q},  $p(w,x,y,z)$ monotonically decreases wrt.
    $2(s_2 + s_3)x^2 + 2(s_1 + s_3)y^2 + 2(s_1 + s_2)z^2$.
    We have
    \begin{equation}
    \footnotesize
    \begin{aligned}
        & x^2 \le w^2 \\
        \Leftrightarrow & 2(s_2 + s_3)x^2 + 2(s_1 + s_3)y^2 + 2(s_1 + s_2)z^2 \le 2(s_2 + s_3)w^2 + 2(s_1 + s_3)y^2 + 2(s_1 + s_2)z^2\\
        \Leftrightarrow & p(w,x,y,z) \ge p(x,w,y,z)
    \end{aligned}
    \end{equation}
    Therefore, $(w^2-x^2)$ and $(p(w,x,y,z) - p(x, w, y,z))$ have the same sign, i.e.,
    \begin{equation}
    \footnotesize
        (w^2-x^2)(p(w,x,y,z) - p(x, w, y,z)) \ge 0
    \end{equation}
    and 
    \begin{equation}
    \footnotesize
        \mathcal{L}(0,1,0,0) \ge \mathcal{L}(1,0,0,0)
    \end{equation}
    % Therefore, $w^2 \ge x^2 \Leftrightarrow p(w,x,y,z) \ge p(x, w, y, z)$
    % and $L(0,1,0,0) \ge L(1,0,0,0).$
    Similarly, $\mathcal{L}(0,0,1,0) \ge \mathcal{L}(1,0,0,0)$ and $\mathcal{L}(0,0,0,1) \ge \mathcal{L}(1,0,0,0)$.
    
    
    Therefore, $\mathcal{L}(1,0,0,0)$ has the minimum value, and $\Bar{\mathbf{q}}=(1,0,0,0)$, $\Bar{\mathbf{R}}'=\mathbf{I}$. 
    
    Finally, considering Eq. \ref{eq:rprime},
    \begin{equation}
    % \footnotesize
        \Bar{\mathbf{R}} = \mathbf{UIV}^T = \mathbf{UV}^T
    \end{equation}
    
\end{proof}

\begin{preliminary}
    Denote the transformation between rotation matrix and unit quaternion as $\mathbf{R}=\gamma(\mathbf{q})$.
    For rotations $\mathbf{R}_1$ and $\mathbf{R}_2$, we have 
    \begin{equation}
    \footnotesize
        \|\mathbf{R}_1 - \mathbf{R}_2\|^2_F = 8(1-\gamma^{-1}(\mathbf{R}_1)^T \gamma^{-1}(\mathbf{R}_2) \gamma^{-1}(\mathbf{R}_2)^T \gamma^{-1}(\mathbf{R}_1))
    \end{equation}
    \label{pre:norm}
\end{preliminary}


\begin{proof}
    Let $\gamma^{-1}(\mathbf{R}_1) = (w_1, x_1, y_1, z_1)$, $\gamma^{-1}(\mathbf{R}_2) = (w_2, x_2, y_2, z_2)$, $\gamma^{-1}(\mathbf{R}_1^T\mathbf{R}_2) = (w', x', y', z')$, then 
    \begin{equation}
    \footnotesize
        \mathbf{R}_1^T \mathbf{R}_2 = \begin{pmatrix} 1-2y'^2-2z'^2 & 2x'y'-2z'w' & 2x'z'+2y'w' \\ 2x'y'+2z'w' & 1-2x'^2-2z'^2 & 2y'z'-2x'w' \\ 2x'z'-2y'w' & 2y'z'+2x'w' & 1-2x'^2-2y'^2 \end{pmatrix}
    \end{equation}

    % \begin{equation}
    % \footnotesize
    %     \| \mathbf{R}_1 - \mathbf{R}_2 \|^2_F = \| \mathbf{R}_1^T (\mathbf{R}_1 - \mathbf{R}_2) \|^2_F = \| \mathbf{I} - \mathbf{R}_1^T\mathbf{R}_2 \|^2_F
    % \end{equation}

    Therefore, 
    \begin{equation}
    \footnotesize
    \begin{aligned}
        \| \mathbf{R}_1 - \mathbf{R}_2 \|^2_F &= \| \mathbf{R}_1^T (\mathbf{R}_1 - \mathbf{R}_2) \|^2_F \\ &= \| \mathbf{I} - \mathbf{R}_1^T\mathbf{R}_2 \|^2_F \\ &= \left\| \mathbf{I} - \begin{pmatrix} 1-2y'^2-2z'^2 & 2x'y'-2z'w' & 2x'z'+2y'w' \\ 2x'y'+2z'w' & 1-2x'^2-2z'^2 & 2y'z'-2x'w' \\ 2x'z'-2y'w' & 2y'z'+2x'w' & 1-2x'^2-2y'^2 \end{pmatrix} \right\|^2_F \\
        & =8(1-w'^2)
    \end{aligned}
    \end{equation}
Since $\mathrm{conj}\left(\gamma^{-1}(\mathbf{R}_1)\right) \times \gamma^{-1}(\mathbf{R}_2)=\gamma^{-1}(\mathbf{R}_1^T\mathbf{R}_2)$, we have 
\begin{equation}
\footnotesize
\begin{aligned}
    w' &= -w_1w_2-x_1x_2-y_1y_2-z_1z_2 \\
    &=-\gamma^{-1}(\mathbf{R}_1)^T \gamma^{-1}(\mathbf{R}_2)
\end{aligned}
\end{equation}
Therefore,
\begin{equation}
\footnotesize
    \begin{aligned}
        &8(1-w'^2) \\
        =& 8(1-(\gamma^{-1}(\mathbf{R}_1)^T\gamma^{-1}(\mathbf{R}_2))^2) \\
        =& 8(1-\gamma^{-1}(\mathbf{R}_1)^T \gamma^{-1}(\mathbf{R}_2) \gamma^{-1}(\mathbf{R}_2)^T \gamma^{-1}(\mathbf{R}_1))
    \end{aligned}
\end{equation}
\end{proof}

We did not find a proper definition of higher order moments under the chordal metrics.

==> response_tex/r1.tex <==
\paragraph{Reviewer1}


\begin{enumerate}
\setlength{\itemsep}{15pt}

\item\textit{The normalizing constant of the matrix Fisher distribution is reduced to one-dimensional integration, and one can construct the derivatives of the normalizing constant that are required for maximum likelihood estimation and moments calculation. As such, the absence of any analytical expression for the normalizing constant is significant drawback. The authors should put more efforts to derive the normalizing constant of the rotational Laplace distribution analytically, and at least, it should be explicitly shown that the normalizing constant depends only on S (which should be straightforward).}


\input{response_tex/math_constant}


\item \textit{As this paper is proposing a new distribution, several fundamental statistical properties should be provided, including mode, mean, and moments. Also, the degree of uncertainties and the shape of the distribution should be interpreted for a given A. Without these information or interpretation, there is no point of performing probabilistic regression.}


Thanks for the suggestions.

% \textbf{Statistical properties.}

\textbf{Mode.} Suppose the proper singular value decomposition of the parameter $\mathbf{A}$ is given by $\mathbf{A}=\mathbf{USV}^T$. 
The \textit{mode} of the distribution is computed as 
\begin{equation}
    \mathbf{R}_0=\mathbf{UV}^T
\end{equation}

% \todo{geodesic mean}
% \todo{moments: no definition}

\input{response_tex/math_mean}




\textbf{Degree of uncertainty}

The degree of uncertainty of rotation Laplace distribution is measured via $\frac{1}{s_i+s_j}$.

As shown in Prop. 2 in the main paper, let $\boldsymbol{\Phi} = \log (\mathbf{R}_0^T\mathbf{R}) \in \mathfrak{so}(3)$ and $\boldsymbol{\phi} = {\boldsymbol{\Phi}^\vee} \in \mathbb{R}^3$. For rotation matrix $\mathbf{R} \in \SO$ following rotation Laplace distribution, when
$\|\mathbf{R} - \mathbf{R}_0\|\rightarrow 0$
, $\boldsymbol{\phi}$ follows zero-mean multivariate Laplace distribution with $\boldsymbol{\Sigma} = 4 \mathbf{V}\operatorname{diag}(\frac{1}{s_2+s_3},\frac{1}{s_1+s_3},\frac{1}{s_1+s_2})\mathbf{V}^T$.
Thus the degree of uncertainty is measured via $\frac{1}{s_i+s_j}$.


\textbf{Shape of the distribution.}

Following the study of matrix Fisher distribution \cite{lee2018bayesian,mohlin2020probabilistic}, we illustrate the impact of $\mathbf{A}$ on the shape of the rotation Laplace distribution in Figure \ref{fig:vis_shape}.
(a) For a diagonal $\mathbf{A}$, the mode of the distribution is identity and the principal axes correspond to $e_1, e_2, e_3$, where the distribution for each axis is circular and identical. (b) For $\mathbf{A}$ with larger singular values, the distribution are more peaked. (c) The distributions for the $x$- axis are more peaked than the $y$- and $z$- axes, since the first singular value dominates. (d,e,f) The parameter $\mathbf{A}$ is obtained by left-multiplying $\mathbf{T}_i$ and right-multiplying $\mathbf{T}_i^T$, where $\mathbf{T}_i$ refers to the rotation matrix by rotating $\pi/4$ around $e_i$. The mode of the distribution is still identity. However, the principal axes vary according to the columns of $\mathbf{A}$. Thus the orientation of the spread has been affected by the direction of the principal axes.


\input{response_tex/fig_vis_distribution}

\jiangran{We incorporate the above properties as Section 4.3 of the revised manuscript.}


\item \textit{Related to the above, it is unclear how the attitude is determined after the matrix parameter A is obtained. There will be issues of uniqueness depending on the values of S, which should be clarified.}

With the parameter $\mathbf{A}$, we determine the mode of the distribution and present it as the output attitude. 
Given a specific parameter $\mathbf{A}$, the proper singular value $\mathbf{S}$ is unique \cite{strang2022introduction}, with the proof in the subsequent paragraph. And thus the probability density function of the distribution, and the mode of the distribution are both unique.

Uniqueness of singular values of matrix $\mathbf{A} \in \mathbb{R}^{m\times n}$: 
Given $\mathbf{AA}^T=\mathbf{U}\boldsymbol{\Sigma}^2\mathbf{U}^T$ and $\mathbf{A}^T\mathbf{A}=\mathbf{V}^T{\Sigma}^2\mathbf{V}$, the singular values of $\mathbf{A}$ can be obtained from the square roots of the eigenvalues of $\mathbf{AA}^T$ or $\mathbf{A}^T\mathbf{A}$, implying uniqueness of the singular values.

% \jiangran{We provide the clarification of distribution mode in the Section 4.3 of the revised manuscript}

\item \textit{While the distribution is motivated to improve robustness against outliers, one noticeable drawback is that it is not smooth near the correct attitude. For example, as shown in Figure 1, the gradient is very large for data with zero error. This may cause numerical issues in training. This should be carefully analyzed.}

Thanks for the advice. Similar to the multivariate Laplace distribution in Euclidean space, rotation Laplace distribution in $\SO$ manifold is also not smooth near the mode. This intrinsic limitation holds for both distributions.

\jiangran{Specifically in regression tasks, when the predicted mode closely approximates the ground truth, the denominator of the function, i.e., $\sqrt{\operatorname{tr}(\mathbf{S} - \mathbf{A}^T\mathbf{R})}$, tends to approach zero. This situation leads to a numerical issue characterized by large gradients.} We address this issue by clipping its probability density function near the mode to prevent numerical problems. Specifically, we clip $\operatorname{tr}(\mathbf{S} - \mathbf{A}^T\mathbf{R})$ in the denominator by $\max(\epsilon, \operatorname{tr}(\mathbf{S} - \mathbf{A}^T\mathbf{R}))$, where $\epsilon=1e-8$.

To assess the robustness of our clipping strategy, we examine the impact of different values for the clipping parameter $\epsilon$. As illustrated in Table \ref{tab:ablation_clip} and Figure \ref{fig:ablation_clip}, our method exhibits similar performance and training processes with different $\epsilon$ values, without encountering numerical issues. These experiments underscore the effectiveness and robustness of our strategy when applying the rotation Laplace distribution to regression tasks.

\jiangran{Compared to our originally submitted version, the above clarification may enhance clarity, leading us to incorporate it into Section 4.5. Additionally, we provide the above discussion about the robustness of the clipping strategy in Section 5.7.}

\begin{table}[t]
    \centering
    \footnotesize
    \caption{\textbf{Ablation study on the clipping parameter $\epsilon$.} The clipping parameter does not affect the results. The experiments are on ModelNet10-SO3 dataset averaged on all categories.}
    \begin{tabular}{ccccccc}
        \toprule
        $\epsilon$ & Acc@3$^\circ$$\uparrow$ & Acc@5$^\circ$$\uparrow$ & Acc@10$^\circ$$\uparrow$ & Acc@15$^\circ$$\uparrow$ & Acc@30$^\circ$$\uparrow$ & Med.($^\circ$)$\downarrow$  \\
        \midrule
         % vRLaplaceProper_clip1e_4 iter623550
        $1\mathrm{e}{-4}$      & 0.450 & 0.614 & 0.718 & 0.743 & 0.769 & 12.8 \\
        $1\mathrm{e}{-8}$      & 0.445 & 0.611 & 0.716 & 0.742 & 0.771 & 13.0 \\
        % vRLaplaceProper_clip1e_12 iter588000
        $1\mathrm{e}{-12}$      & 0.441 & 0.608 & 0.714 & 0.742 & 0.769 & 12.5 \\
        \bottomrule
    \end{tabular}
    \label{tab:ablation_clip}
\end{table}


\input{response_tex/fig_clip_curve}




\item \textit{It is suggested to perform a benchmark study for a simple estimation problem, such as the Wahba’s problem that commonly appear in the referenced papers. Especially, those papers present the training process, i.e., the reduction of the loss function or the test error over the course of iterations to compare numerical properties.}

Thanks for the suggestion. We benchmark our method on the Wahba's problem.

\begin{problem} \textbf{Wahba's Problem}

Given two sets of n points $\{ p_1, p_2, ..., p_n\}$ and $\{ p_1^*, p_2^*, ..., p_n^*\}$, where $n\ge 2$, find the rotation matrix $\mathbf{R}$ which brings the first set into the best least squares coincidence with the second. That is, find $\mathbf{R}$ which minimizes
\begin{equation}
    \sum_{i=1}^{n} \| p_i^* - \mathbf{R}p_i\|^2
\end{equation}
\end{problem}

In accordance with the methodology outlined in \cite{zhou2019continuity, peretroukhin2020smooth}, our neural network is trained on 2290 airplane point clouds from ShapeNet dataset \cite{shapenet2015}. Subsequently, testing is conducted on 400 held-out point clouds. Throughout both training and evaluation phases, each point cloud undergoes a random rotation. The training process involves 10,000 iterations utilizing the Adam optimizer, with a batch size of 100. We experiment with different learning rates.

The progress of training and test errors across iterations is visually depicted in Figure \ref{fig:wahba}. Notably, rotation Laplace distribution achieves superior or comparable performances with alternative rotation representations or distributions.
% consistently outperforms alternative rotation representations or distributions.


\jiangran{We add these experiments on Wahba's Problem as Section 5.9 in the revised manuscript.}

\input{response_tex/fig_wahba}


% \todo{wahba}


\item \textit{Related to the above comment, the authors should consider the case of very large uncertainties, i.e., S is close to zero.}


\jiangran{In rotation regression tasks, when the predicted $\mathbf{S}$ approaches zero, the denominator of probabilistic function, i.e., $\sqrt{\operatorname{tr}(\mathbf{S} - \mathbf{A}^T\mathbf{R})}$ equals zero. To effectively address this numerical problem, we employ the clipping strategy outlined in Question 4 which ensures a stable training process.}

%In the experiments of Wahba's problem, most of the instances exhibit really small certainties, with $s_1, s_2, s_3$ vary from \todo{xx} to xx, xx to xx, xx to xx, respectively. We hypothesis the main reason is that the task is relatively simple.
% \todo{We can evaluate the uncertainty with $\frac{s_1}{\mathbf{E}(s_1)}$ and $\frac{\sqrt{s_2+s_3}}{\sqrt{s_1+s_2}}$.}

% \begin{proof}

% Whether the model exhibits a comparable level of certainty in at least one direction of a particular output, as in other outputs, can be expressed by $\frac{s_1}{\mathbf{E}(s_1)}$.

% To evaluate whether the model is certain to all directions of a particular output, we need to calculate the probabilistic density function.

% Let $R$ represent the rotation whose rotation angle is $\theta$ and rotation axis is $k=(k_x,k_y,k_z)$, then $R$'s matrix form can be written as:

% \begin{equation*}
%     \footnotesize
%     R(k,\theta)=\begin{pmatrix} \cos{\theta}+k_x^2(1-\cos{\theta}) & -\sin{\theta}k_z+(1-\cos{\theta})k_xk_y & \sin{\theta}k_y+(1-\cos{\theta}) \\ \sin{\theta}k_z+(1-\cos{\theta})k_xk_y & \cos{\theta}+k_y^2(1-\cos{\theta}) & -\sin{\theta}k_x+(1-\cos{\theta})k_yk_z \\
%     -\sin{\theta}k_y+(1-\cos{\theta})k_xk_z& \sin{\theta}k_x+(1-\cos{\theta})k_yk_z & \cos{\theta}+k_z^2(1-\cos{\theta}) \end{pmatrix}
% \end{equation*}    

% So if we fix the rotation angle $\theta$ of $\mathbf{R}'=\mathbf{U}^T\mathbf{R}\mathbf{V}$ and change the rotation axis $k$ of $\mathbf{R}'$, the probability density function can be maximized when $|k_z|=1$, and minimized when $|k_x|=1$.

% If we fix $s_1,s_2,s_3$, then the probability density function is proportional to $\frac{\exp\left(-\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{R}')}\right)}{\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{R}')}}$. When $|k_z|=1$, it can be expanded as $\frac{\sqrt{2}}{\sqrt{s_1+s_2}\theta}-1+O(\theta)$ around $\theta=0$, and when $|k_x|=1$, it can be expanded as $\frac{\sqrt{2}}{\sqrt{s_2+s_3}\theta}-1+O(\theta)$. Thus the ratio $\frac{\sqrt{s_2+s_3}}{\sqrt{s_1+s_2}}$ can be used to evaluate whether the model is uncertain in some directions while certain in other directions.

% \end{proof}

% \todo{In the experiments of Wahba's problem, most of the instances exhibit really small uncertainties, with $\frac{s_1}{\mathbf{E}(s_1)}$ vary from 0.81 to 1.38 and $\frac{\sqrt{s_2+s_3}}{\sqrt{s_1+s_2}}$ vary from 0.56 to 0.79. We hypothesize the main reason is that the task is relatively simple.
% }

% For Wahba's problem, we assume correspondences of around a thousand points of two airplanes. Considering three non-coplanar points decide the target rotation, this task is relatively simple and deterministic. And in experiments, we did not observe significant differences in the uncertainty across different cases.


To better study our distribution in the circumstances of large uncertainties, we analyze several cases in Pascal3D+ dataset, with very large uncertainties, shown in Table \ref{tab:large_uncertainties}.
\input{response_tex/tab_large_uncertainties}

We see that the instances exhibit 
% one large singular value and two 
small singular values due to (near) symmetry or poor image quality, also leading to large prediction errors. 
% When $\mathbf{S}$ is close to zero, the distribution is close to a uniform distribution, and there is no numerical issues.


% \todo{
% we did not find an instance with very large uncertainties. The abs values of $s_1, s_2, s_3$ vary from $xx to xx, xx to xx, xx to xx$, where most of the instance exhibit really certainties. We hypothesis it is because the task is relatively simple.
% } 

% \todo{
% Haoran: Evaluate table1 and find 5 cases with the largest uncertainty, find the input image and the predicted A. 

% For experiments in ModelNet10-SO3 dataset (Table 1 in the paper), we find two cases with the largest uncertainty.  Input image, A, S, error; Reason: symmetry. Uncertainty -> performance. No numerical issues.
% }



\item \textit{It is hard to believe that the rotational Laplace distribution outperforms all of the other approaches for every case considered. In deep learning, there is a reason why the Gaussian distribution is popular. There should be candid efforts to illustrate its benefits and limitations precisely.}

% \todo{Say something good to Gaussian. We acknowledge the pros of Gaussians. We did not mean to replace Gaussian, just a complementary distribution.}

While rotation Laplace distribution offers advantages in robustness against the disturbance of outlier data, it is subject to several limitations.


Primarily, the probability density function of our distribution is relatively complex, which poses a significant challenge in deriving an analytical solution for the normalization factor and may limit its applicability across various downstream tasks.
% \jiangran{Primarily, the probability density function of our distribution is relatively complex, which poses a significant challenge in deriving an analytical solution for the normalization factor. Although this characteristic does not affect its applicability across various downstream deep-learning tasks, the discontinuity may constrain further derivations and research efforts.}
% and certain statistical properties. \todo{This complexity limits its applicability across various downstream tasks. however, don't affect}
Moreover, due to the existence of the denominator in the probability density function, rotation Laplace distribution may exhibit numerical issues in training when the predicted mode is near the ground truth or the predicted $\mathbf{S}$ is near zero. Additional operations, e.g., clipping the denominator, are required to address the issues.
\yingda{Refining the computation of the normalization constant or introducing a more elegant form of distribution can be important future directions.}

% Moreover, the probability density function exhibits non-smooth behavior near the mode, resulting in a singularity. This singularity gives rise to large gradients in proximity to the mode, necessitating specific design considerations, i.e. clipping, for numerical stability. \todo{S turns zero, numerical issue}
% Furthermore, deriving an analytical solution for the normalization factor of the rotational Laplace distribution poses a considerable challenge, making it less applicable for various downstream tasks.

% \todo{Math properties not elegant}

\yingda{
Gaussian distribution is the most popular distribution in deep learning and has withstood the test of time. Its mathematical properties are exceptionally good, making it highly effective across a wide range of tasks. With the introduction of rotation Laplace distribution, we do not aim to replace Gaussian distribution or matrix Fisher distribution but rather to provide a supplementary alternative for users.
}

\jiangran{We add the above analysis of limitation as Section 10 in the revised manuscript.}

% \jiangran{we do not aim to replace the Gaussian distribution or matrix Fisher distribution}

\end{enumerate}

==> response_tex/r2.tex <==
\paragraph{Reviewer2}


\begin{enumerate}
\setlength{\itemsep}{15pt}

\item \textit{The current experiments are conducted on ModelNet10-SO3 and Pascal3D+. It is recommended to include the more commonly used benchmarks like LINEMOD and YCB video datasets to better compare with the state-of-the-art methods.}


\jiangran{Thanks for the valuable advice.
6DoF object pose estimation emerges as a significant downstream task for our proposed rotation representation. This task involves estimating the 3D translation and 3D rotation of an object from a single RGB image, with broad applications in real-world tasks such as robotic manipulation, augmented reality, and autonomous driving. Leveraging the inherent nature of probabilistic modeling, rotation Laplace distribution can seamlessly integrate into existing regression-based methods. We conduct experiments using GDR-Net \cite{wang2021gdr} as the baseline to showcase the advantages of incorporating our method. 

\input{response_tex/6dpose_detail}

We add the above content in the manuscript as Section 8.
}

\item \textit{The proposed approach involves several mathematical concepts and computations. Maybe this should not be regarded as a weakness but it may indeed make it difficult to implement or apply in practice.  But I am glad to see the code has been released.}


To apply the rotation Laplace distribution in downstream tasks, the only requirement is a function that takes the parameter $\mathbf{A}$ as input and outputs the probability density function $p(\mathbf{R})$, which is included in the released code.

In this paper, we include detailed derivations and proofs mainly to elucidate our design concept and establish the robust connections between the rotation Laplace distribution in the $\SO$ manifold and the multivariate Laplace distribution in Euclidean space.




\item \textit{In the multi-modal prediction part, it is claimed that the multi-modal prediction is helpful in handling symmetric objects. Some previous methods also adopted some other types of symmetry-aware loss functions to handle the symmetry \cite{wang2021gdr}. Could you further compare your method with them and discuss the advantages of your method?}


As suggested, we experimented with the min-of-N loss adopted in GDR-Net \cite{wang2021gdr}.
The min-of-N loss considers the set of all possible ground truth rotations under symmetry and supervises the network prediction by selecting the ground truth with the minimum error, defined as:
\begin{equation}
    \mathcal{L}_{\text{min-of-N}} = \min_{\mathbf{R}\in\mathcal{R}} \mathcal{L}(\hat{\mathbf{R}}, \mathbf{R})
\end{equation}
where $\hat{\mathbf{R}}$ and $\mathbf{R}$ denote the prediction and the ground truth, respectively.


In our case, we manually compute the set of possible ground truths for symmetric objects. Specifically, we assume 2-symmetry for \texttt{bathtub}, \texttt{desk}, \texttt{dresser}, \texttt{night-stand} and \texttt{table} categories of ModelNet10-SO3 dataset.
\yingda{Due to the absence of object CAD models in our category-level rotation regression tasks, instead of min-of-N Point-Matching loss in \cite{wang2021gdr}, we experiment with min-of-N NLL loss.}
We compare the min-of-N loss and our multi-modal distribution in Table \ref{tab:min-of-N}.
For min-of-N loss, we report the better performance between the prediction and the two possible ground truths for symmetric objects. Similarly, for multi-modal distribution, we report the better result of the top-2 predictions.

\begin{table*}[t]
  \centering
  \footnotesize
  \caption{\small Numerical comparisons with different methods to handle symmetry. The experiments are on ModelNet10-SO3 dataset averaged on all categories.}
    \begin{tabular}{lccc}
    \toprule
          & Acc@15$^\circ$$\uparrow$ & Acc@30$^\circ$$\uparrow$ & Med.($^\circ$)$\downarrow$  \\
    \midrule
    Min-of-N loss              &  0.844 & 0.874 & 3.1       \\
    % vRLaplaceProper_release 543000
    Multi-modal distribution              & \textbf{ 0.900}  &  \textbf{0.918} &  \textbf{2.3}         \\
    \bottomrule
    \end{tabular}%
  \label{tab:min-of-N}%
\end{table*}%

As depicted in the results, our multi-modal distribution consistently outperforms the min-of-N loss when handling symmetric objects. Moreover, in contrast to the min-of-N loss, which necessitates knowledge of the symmetry pattern to obtain all possible ground truths before training, the multi-modal distribution automatically generates different modes for ambiguous inputs from the data.

\jiangran{We incorporate the above results and discussion in the revised manuscript as Section 9.3.4. }

\item \textit{Could you explain more about Fig.10? Does each column demonstrate a modal of the mixture model?}


Yes, \jiangran{your understanding is completely correct.} Given our configuration of the mixture model with four modes, the visualizations are distributed across the four columns. The solid circles denote the ground truths. 

\jiangran{We incorporate the above clarification in the Section 9.3.3 of revised manuscript.}


\item \textit{There are some typos.}

Thanks for the detailed comments. We have proofread the manuscript carefully and fixed the typos and other writing issues.



\end{enumerate}

==> response_tex/r3.tex <==
\paragraph{Reviewer3}


\begin{enumerate}
\setlength{\itemsep}{15pt}

\item \textit{The paper uses numerical integration to compute the normalization factor, and it uses 37K samples. What are the results when using fewer and more samples. Does the discretization strategy matter?}

To investigate the impact of the computation of the normalization factor, we conduct an ablation study on the number of quantizing grids using the ModelNet10-SO(3) toilet category dataset, shown in Table \ref{tab:num_sample}. 

We applied uniform sampling over $\SO$ manifold as in \cite{murphy2021implicit}. The number of samples starts at 72 and iteratively grows by a factor of 8, resulting in $72 \times 8^l$ samples. We explore values for $l$ ranging from 0 to 4. 
To better evaluate the impact of different sampling strategies, we also measure the forward and backward time for one pass of a batch of 32 instances on a single 3090 GPU.



\begin{table}[t]
    \centering
    \footnotesize
    \caption{\small \textbf{Ablation studies on the impact of the number of samples for the normalization factor.} The experiments are on ModelNet10-SO(3) toilet category dataset.}
    \begin{tabular}{lccccc}
        \toprule
        \#grids & Mean ($^\circ$)$\downarrow$ & Median ($^\circ$)$\downarrow$ & Acc@5$^\circ$$\uparrow$ & Forward time (ms) & Backward time (ms) \\
        \midrule
        72 $(l=0)$      & 6.0 & 3.2 & 0.76 & 2.3 & 0.7 \\
        576 $(l=1)$     & 5.8 & 2.8 & 0.80 & 2.3 & 0.7 \\
        4608 $(l=2)$    & 5.3 & 2.6 & 0.82 & 2.7 & 0.8 \\
        36864 $(l=3)$   & 5.2 & 2.6 & 0.82 & 5.1 & 1.7 \\
        294912 $(l=4)$  & 5.3 & 2.5 & 0.82 & 26.4 & 12.9 \\
        \bottomrule
    \end{tabular}
    \label{tab:num_sample}
\end{table}


Table \ref{tab:num_sample} illustrates that using too few grid samples leads to inferior performance, and increasing the number of samples results in better performance at the cost of longer runtime. The performance improvement saturates when $l \ge 2$. After considering both performance and computational efficiency, we choose 37K samples as a balanced option.

\jiangran{We add this ablation study in the revised manuscript as Section 5.7.}


\item \textit{How does the quaternion representation compare against the matrix-based representation across all the experiments.}

\jiangran{We evaluate the performance of quaternion Laplace distribution across all rotation regression benchmarks.} As shown in Table \ref{tab:q1}, \ref{tab:q2}, \ref{tab:q3} and \ref{tab:q4}, rotation Laplace distribution consistently achieves superior performance than quaternion Laplace distribution. 

\jiangran{We present the results in Section 5 of the revised manuscript.}

\input{response_tex/tab_quaternion}



\item \textit{How about extending SO(3) to SE(3)? Many pose estimations for 6D.}


\jiangran{

We appreciate the valuable suggestion.
In specific, we extend our method to the 6DoF object pose estimation task. This task involves estimating the 3DoF translation and 3DoF rotation of an object from a single RGB image, with broad applications in real-world tasks such as robotic manipulation, augmented reality, and autonomous driving. Leveraging the inherent nature of probabilistic modeling, rotation Laplace distribution can seamlessly integrate into existing regression-based methods. We conduct experiments using GDR-Net \cite{wang2021gdr} as the baseline to showcase the advantages of incorporating our method. 


\input{response_tex/6dpose_detail}

We incorporate above content as Section 8 of the revised manuscript.

}

\end{enumerate}

==> response_tex/tab_large_uncertainties.tex <==
\begin{table}[t]
    \centering
    % \footnotesize
    \small
    \caption{\textbf{Instances with large uncertainties in Pascal3D+.} The table includes the input image, the predicted singular values, and the prediction errors.}
    \begin{tabular}{m{3cm}m{3cm}m{3cm}m{3cm}}
    \toprule
        Input image
        & \centering \includegraphics[width=0.6\linewidth]{figures/response/528.jpg}
        & \centering \includegraphics[width=0.6\linewidth]{figures/response/253.jpg}
        & \centering \includegraphics[width=0.6\linewidth]{figures/response/1555.jpg} \tabularnewline
    \midrule
        Singular values $\mathbf{S}$ &  \centering  71, 0.26, 0.14 &  \centering 1778, 1.6, 0.69 & \centering  427, 1.5, 0.079 \tabularnewline
    \midrule
        Prediction error ($^\circ$) & \centering 179.5 & \centering 179.6 & \centering 70.5 \tabularnewline
    \bottomrule
        
    \end{tabular}
    \label{tab:large_uncertainties}
\end{table}

==> response_tex/tab_quaternion.tex <==
\begin{table*}[t]
  \centering
  \footnotesize
  \caption{\small Numerical comparisons with probabilistic baselines on ModelNet10-SO3 dataset averaged on all categories.}
    \begin{tabular}{lcccccc}
    \toprule
          & Acc@3$^\circ$$\uparrow$ & Acc@5$^\circ$$\uparrow$ & Acc@10$^\circ$$\uparrow$ & Acc@15$^\circ$$\uparrow$ & Acc@30$^\circ$$\uparrow$ & Med.($^\circ$)$\downarrow$  \\
    \midrule
    % QLaplace_current VLamVT iter361.7k
    quaternion Laplace              &  0.242  &  0.469 &  0.647  &  0.692  & 0.741  &  18.3   \\
    % vRLaplaceProper_release 543000
    rotation Laplace                &  \textbf{0.445}  & \textbf{0.611}  &  \textbf{0.716}  &  \textbf{0.742}  &  \textbf{0.771} & \textbf{13.0}   \\
    \bottomrule
    \end{tabular}%
  \label{tab:q1}%
\end{table*}%



\begin{table*}[t]
  \centering
  \footnotesize
  \caption{\small Numerical comparisons with probabilistic baselines on Pascal3D+ dataset averaged on all categories.}
    \begin{tabular}{lcccccc}
    \toprule
          & Acc@3$^\circ$$\uparrow$ & Acc@5$^\circ$$\uparrow$ & Acc@10$^\circ$$\uparrow$ & Acc@15$^\circ$$\uparrow$ & Acc@30$^\circ$$\uparrow$ & Med.($^\circ$)$\downarrow$  \\
    \midrule
    % vsynth_both_pascal_RLaplaceProper_release1 state_dict_806000
    quaternion Laplace              & 0.125   & 0.252  &   0.502 & 0.648   & 0.834  &   11.4  \\
    rotation Laplace                 &  \textbf{0.134} & \textbf{0.292} & \textbf{0.574}  &  \textbf{0.714}  & \textbf{0.874} &  \textbf{9.3}  \\
    \bottomrule
    \end{tabular}%
  \label{tab:q2}%
\end{table*}%

{
\setlength{\tabcolsep}{5pt}
\begin{table*}[t]
    \caption{\small Numerical comparisons with our proposed quaternion \& rotation Laplace distributionon ModelNet10-SO3 dataset. One model is trained for each category.}
    \vspace{2mm}
    \centering
    \scriptsize
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{}&& Chair &&&Sofa&&& Toilet&&&Bed&\\
    \cmidrule{2-13}  
        & Mean$\downarrow$ & Med.$\downarrow$ & Acc@5$\uparrow$ 
        & Mean$\downarrow$ & Med.$\downarrow$ & Acc@5$\uparrow$ 
        & Mean$\downarrow$ & Med.$\downarrow$ & Acc@5$\uparrow$ 
        & Mean$\downarrow$ & Med.$\downarrow$ & Acc@5$\uparrow$ 
        \\
        \midrule
        % chair:543k, sofa:343.5k, toilet:597k, bed:573k
        quat. Laplace & 12.6 & 5.2 & 0.49 & 13.1 & 3.7 & 0.67 & 5.9 & 3.4 & 0.69 & 17.7 & 3.4 & 0.69\\
        rot. Laplace & \textbf{9.7}  & \textbf{3.5}  &  \textbf{0.68} & \textbf{8.8} & \textbf{2.1} & \textbf{0.84}  & \textbf{5.3} & \textbf{2.6} & \textbf{0.83} & \textbf{15.5} & \textbf{2.3} & \textbf{0.82}  \\
        % RLaplace-RPMG code base & {11.0}  & {4.0}  &  {0.61} & {10.0} & {2.3} & {0.82}  & {7.6} & {3.0} & {0.76} & {18.6} & {3.0} & {0.76}  \\
        \bottomrule
    \end{tabular}
  \label{tab:q3}
\end{table*}
}



{
\setlength{\tabcolsep}{8pt}
\begin{table*}[h]
  \centering
  \scriptsize
    % \fontsize{6}{7}\selectfont
      \caption{\small Numerical comparisons on Pascal3D+ dataset. One model is trained for each category.}
      \vspace{2mm}
    \begin{tabular}{l|cccc|cccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[4]{*}{Methods}} & \multicolumn{4}{c|}{Bicycle}  & \multicolumn{4}{c}{Sofa} \\
\cmidrule{2-9}          & Acc@10$\uparrow$ & Acc@15$\uparrow$ & Acc@20$\uparrow$ & Med.$\downarrow$  & Acc@10$\uparrow$ & Acc@15$\uparrow$ & Acc@20$\uparrow$ & Med.$\downarrow$ \\
    \midrule
    quat. Laplace        &   0.398  &  0.559  & 0.686  & 12.2  &   0.615 &   0.769 & 0.923 & 8.4   \\
    % bicycle: point533, sofa: point441
    rot. Laplace        &  \textbf{0.435}   &   \textbf{0.641}&  \textbf{0.744}&   \textbf{11.2}&   \textbf{0.735}&    \textbf{0.900}&     \textbf{0.964}&  \textbf{6.3} \\
    \bottomrule
    \end{tabular}%
  \label{tab:q4}%
\end{table*}%
}

==> revision2/mode_uniqueness.tex <==
% \section{Comment1}
\textit{Regarding responses 2 and 3, the mean attitude or mode given by (16) may not be unique depending on the singular values. For example, when all of the singular values are zero, there are three degrees of freedom in the mode, or it is completely undefined. As such, even though the singular values are unique, the mode might not be unique. There are several other cases where the mode is not unique, and those should be properly discussed in the manuscript.}

Thanks for pointing out. 
The mode of our distribution may not be unique depending on the singular values. The detailed study is shown as below:

For rotation Laplace distribution
\begin{equation}
    p(\mathbf{R}; \mathbf{A})
    = \frac{1}{F(\mathbf{A})} \frac{\exp\left(-\sqrt{\operatorname{tr}\left(\mathbf{S} - \mathbf{A}^T \mathbf{R}\right)}\right)}
    {\sqrt{\operatorname{tr}\left(\mathbf{S} -\mathbf{A}^T \mathbf{R}\right)}},
\end{equation}
let $s_1, s_2, s_3$ be the proper singular values of the parameter $\mathbf{A}$,
the mode of the distribution is computed as
\begin{equation}
    \mathbf{R}_0 = \begin{cases} 
        \mathbf{UV}^T, &  \text{case1: }s_2 + s_3 > 0 \\ 
        \mathbf{U} \left(\begin{smallmatrix} 1 & 0 & 0 \\ 0 & 1-2x^2 & -2xw \\ 0 & 2xw & 1-2x^2 \end{smallmatrix}\right) \mathbf{V}^T, &  \text{case2: }s_2+s_3=0, s_1+s_3>0 \\
        \mathbf{U} \left(\begin{smallmatrix} 1-2y^2 & 2xy & 2yw \\ 2xy & 1-2x^2 & -2xw \\ -2yw & 2xw & 1-2x^2-2y^2 \end{smallmatrix} \right) \mathbf{V}^T, & 
        \text{case3: }s_2+s_3=0, s_1+s_3=0, s_1+s_2>0 \\
        \text{ill-defined}, & \text{case4: }s_2+s_3=0, s_1+s_3=0, s_1+s_2=0
\end{cases}
\end{equation}
where $\mathbf{q}'=(w, x, y, z)$ is the corresponding unit quaternion of the rotation matrix $\mathbf{U}^T\mathbf{RV}$ (see Eq.\ref{eq:r_to_q}).

With the help of the visualization method \cite{murphy2021implicit}, we show the modes in different cases in Figure \ref{fig:unique_vis}.

% \yingda{We noticed that matrix Fisher distribution has the similar mode uniqueness property with ours.}

\begin{figure*}[h]
    \centering
    \begin{tabular}{ccc}
    \includegraphics[width=0.3\linewidth]{figures/response2/unique1.jpg}
    &\includegraphics[width=0.3\linewidth]{figures/response2/unique2.jpg}
    &\includegraphics[width=0.3\linewidth]{figures/response2/unique3.jpg}
    \\
    \small{case1: $\mathbf{A}=\operatorname{diag}(1, 1, 1)$} &
    \small{case2: $\mathbf{A}=\operatorname{diag}(1, 0, 0)$} &
    \small{case3: $\mathbf{A}=\operatorname{diag}(1, 1, -1)$}
    \\    
    \end{tabular}
    \caption{\small \textbf{Visualization of the modes of rotation Laplace distribution with different parameters.} We use the visualization method in \cite{murphy2021implicit}.}
    \label{fig:unique_vis}
\end{figure*}

% \todo{Fisher also has the same problem.}

\begin{proof}
    For rotation Laplace distribution
    \begin{equation}
    \footnotesize
    \begin{aligned}
        p(\mathbf{R}; \mathbf{A}) 
        &= \frac{1}{F(\mathbf{A})} \frac{\exp\left(-\sqrt{\operatorname{tr}\left(\mathbf{S} - \mathbf{A}^T \mathbf{R}\right)}\right)}
        {\sqrt{\operatorname{tr}\left(\mathbf{S} -\mathbf{A}^T \mathbf{R}\right)}} \\ 
        & = \frac{1}{F(\mathbf{A})} \frac{\exp\left(-\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{U}^T\mathbf{R}\mathbf{V})}\right)}{\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{U}^T\mathbf{R}\mathbf{V})}} \\
        & \xlongequal{\mathbf{R}'=\mathbf{U}^T\mathbf{R}\mathbf{V}}  \frac{1}{F(\mathbf{A})} \frac{\exp\left(-\sqrt{\operatorname{tr}\left(\mathbf{S} - \mathbf{S}\mathbf{R}'\right)}\right)}
        {\sqrt{\operatorname{tr}\left(\mathbf{S} -\mathbf{S}\mathbf{R}'\right)}} 
    \end{aligned}
    \end{equation}

    
    Below we first consider the mode of  $\mathbf{R}'$, denoted as ${\mathbf{R}_0}'$, and then the mode of $\mathbf{R}$ is given as
    \begin{equation}
        {\mathbf{R}_0} = \mathbf{U}{\mathbf{R}}_0'\mathbf{V}^T
        \label{eq:rprime}
    \end{equation}


    
    % We consider the simple case when $\mathbf{A}=\mathbf{S}$. Otherwise, we apply a transformation $\mathbf{R}'=\mathbf{V}^T\mathbf{R}\mathbf{U}$, such that the distribution follows the simple case.
    
    % Given $\mathbf{R}'=\mathbf{U}^T\mathbf{R}\mathbf{V}$, and c
    Considering the transformation $\gamma$ between rotation matrix and unit quaternion
    \begin{equation}
    \footnotesize
        \mathbf{R}' = \gamma(\mathbf{q'}) = \begin{pmatrix} 1-2y^2-2z^2 & 2xy-2zw & 2xz+2yw \\ 2xy+2zw & 1-2x^2-2z^2 & 2yz-2xw \\ 2xz-2yw & 2yz+2xw & 1-2x^2-2y^2 \end{pmatrix},
    \label{eq:r_to_q}
    \end{equation}
    we have 
    % $\mathbf{R}'=\gamma(w, x, y, z)$, then
    \begin{equation}
    \footnotesize
        p(w,x,y,z;\mathbf{A}) = \frac{1}{F(\mathbf{A})} \frac{\exp\left(
        -\sqrt{2(s_2+s_3) x^2 + 2(s_1+s_3) y^2 + 2(s_1+s_2)z^2}
        \right)}{\sqrt{2(s_2+s_3) x^2 + 2(s_1+s_3) y^2 + 2(s_1+s_2)z^2}}
        \label{eq:pdf_q}
    \end{equation}

    Therefore, $p(w,x,y,z)$ monotonically decreases wrt.
    $2(s_2 + s_3)x^2 + 2(s_1 + s_3)y^2 + 2(s_1 + s_2)z^2$.
    % Since $2(s_2 + s_3)x^2 + 2(s_1 + s_3)y^2 + 2(s_1 + s_2)z^2 \ge 0$, 
    Since
    \begin{equation}
        s_1 + s_2 \ge s_1 + s_3 \ge s_2 + s_3 \ge 0,
        \label{eq:property_svd}
    \end{equation}
    we have 
    \begin{equation}
    \begin{aligned}
        & \mathbf{R}' \text{ is mode } 
        \Leftrightarrow 
         (s_2 + s_3)x^2 = 0 \text{ and } (s_1 + s_3)y^2 = 0 \text{ and } (s_1 + s_2)z^2 = 0        
    \end{aligned}
    \end{equation}

    We discuss the values of $s_1 + s_2, s_1 + s_3, s_2 + s_3$ to determine the mode of the distribution.
    
    \begin{itemize}
    \item \textbf{Case 1: } $s_2+s_3>0$ \\
    According to Eq. \ref{eq:property_svd},
    \begin{equation}
    \begin{aligned}
        & \mathbf{R}' \text{ is mode } 
        \Leftrightarrow 
         x = 0 \text{ and } y = 0 \text{ and } z = 0        
    \end{aligned}
    \end{equation}
    Therefore, ${\mathbf{R}_0}' = \mathbf{I}$ is the unique mode for $\mathbf{R}'$, and ${\mathbf{R}_0} = \mathbf{U}\mathbf{V}^T$ is the unique mode for $\mathbf{R}$.
    
    \item \textbf{Case 2: } $s_2+s_3=0$, but $s_1+s_3>0$ \\
    We have
    \begin{equation}
    \begin{aligned}
        & \mathbf{R}' \text{ is mode } 
        \Leftrightarrow 
         y = 0 \text{ and } z = 0        
    \end{aligned}
    \end{equation}
    Therefore, given Eq. \ref{eq:r_to_q}, the modes of $\mathbf{R}'$ are 
    \begin{equation}
    \footnotesize
        \begin{pmatrix} 1 & 0 & 0 \\ 0 & 1-2x^2 & -2xw \\ 0 & 2xw & 1-2x^2 \end{pmatrix},
    \end{equation}
    and the modes of $\mathbf{R}$ have the form of 
    \begin{equation}
    \footnotesize
        \mathbf{U} \begin{pmatrix} 1 & 0 & 0 \\ 0 & 1-2x^2 & -2xw \\ 0 & 2xw & 1-2x^2 \end{pmatrix} \mathbf{V}^T,
    \end{equation} 

    
    \item \textbf{Case 3: } $s_2+s_3=0$, $s_1+s_3=0$, but $s_1+s_2>0$ \\
    We have
    \begin{equation}
    \begin{aligned}
        & \mathbf{R}' \text{ is mode } 
        \Leftrightarrow 
         z = 0        
    \end{aligned}
    \end{equation}

    Therefore, given Eq. \ref{eq:r_to_q}, the modes of $\mathbf{R}'$ are 
    \begin{equation}
    \footnotesize
        \begin{pmatrix} 1-2y^2 & 2xy & 2yw \\ 2xy & 1-2x^2 & -2xw \\ -2yw & 2xw & 1-2x^2-2y^2 \end{pmatrix},
    \end{equation}
    and the modes of $\mathbf{R}$ have the form of 
    \begin{equation}
    \footnotesize
        \mathbf{U} \begin{pmatrix} 1-2y^2 & 2xy & 2yw \\ 2xy & 1-2x^2 & -2xw \\ -2yw & 2xw & 1-2x^2-2y^2 \end{pmatrix}\mathbf{V}^T,
    \end{equation} 


    \item \textbf{Case 4: } $s_2+s_3=0$, $s_1+s_3=0$, $s_1+s_2=0$
    
    We have $s_1=s_2=s_3=0$, therefore, the denominator of $p(w,x,y,z)$ is zero for all $(w,x,y,z)$ and the distribution is ill-defined.
    
    \end{itemize}

\end{proof}

We reclaim the mode in the revised manuscript and include the discussion on uniqueness in the supplementary. 

==> revision2/singularity_exp.tex <==
% \section{Comment2}

\textit{The fundamental drawback of the proposed distribution is singularities appearing in two cases: when the predicted mode is close to the ground truth, and when the uncertainties are large such that S becomes close to zero. While the authors addressed these simply by clipping, the implications of these inherent singularities are not properly illustrated, which may give the impression that the given benchmark examples are handcrafted. I don’t think the proposed distribution should outperform other alternative formulations always. It is suggested to conduct an additional honest benchmark study to show the potential issues of these two types of singularities more clearly.}



\yingda{Thank you for your insightful suggestion. We acknowledge that a notable limitation of our rotation Laplace distribution is the singularities appearing when $\mathbf{S}$ is close to zero and when the predicted mode is close to the ground truth.
To comprehensively illustrate the implications of these singularities, we have conducted targeted experiments, as elaborated below.
\begin{itemize}
    \item \textbf{Singularity 1:} 
    When $\mathbf{S}$ is close to zero, the distribution becomes ill-defined, leading to difficulties in fitting distributions with very large uncertainties, such as the uniform distribution.
    In our experiment, we compare the matrix Fisher distribution and our rotation Laplace distribution in fitting a uniform distribution on SO(3). Specifically, we sampled rotations uniformly over the SO(3) manifold and optimize the parameters of both distributions via negative log likelihood (NLL) loss. We randomly sample a batch of 16 rotations on the fly and optimize over 10k iterations for each distribution.

    After convergence, we uniformly sample 100k samples as the test set. The test NLL loss for the matrix Fisher distribution is 0.0001, while for the rotation Laplace distribution, it is 0.0677. We further visualize the statistical histogram for the probability density of the test set, as illustrated in Fig. \ref{fig:uniform_fit}. 
    Compared to the matrix Fisher distribution, the rotation Laplace distribution exhibit a biased distribution, indicating its inadequacy in representing a uniform distribution. This result highlights the limitation that the rotation Laplace distribution is unsuitable for data that closely follows a uniform distribution.
    
    \begin{figure*}[th]
        \centering
        \begin{tabular}{cc}
        \includegraphics[width=0.45\linewidth]{figures/response2/uniform_fit_fisher_73_2.pdf} &
        \includegraphics[width=0.45\linewidth]{figures/response2/uniform_fit_laplace_73_2.pdf}
        \end{tabular}
        \caption{\textbf{Histogram visualization of the probability density of fitting a uniform distribution.} We let the matrix Fisher distribution and rotation Laplace distribution to fit a uniform distribution, and visualize the probability density function after convergence.}
        \label{fig:uniform_fit}
    \end{figure*}

    \item \textbf{Singularity 2:} 
    When the predicted mode is close to the ground truth, the probability density tends to become infinite, leading to numerical issues. We adopt a clipping strategy to address this problem. However, a remaining issue is the large gradient for predictions with tiny errors, which may result in unstable training.

    To highlight this problem, we conduct an experiment where the matrix Fisher distribution and the rotation Laplace distribution are used to optimize a single rotation, or in other words, to fit a Dirac distribution. Specifically, we use NLL loss and the gradient descent optimizer. The clipping parameter is set as $\epsilon=1e-8$. The optimization curves and results are shown in Fig. \ref{fig:dirac}.
    
    For the rotation Laplace distribution, when the predicted mode $\mathbf{R}_0$ is very close to the ground truth, the probability density function is clipped by $\max(\epsilon, \operatorname{tr}(\textbf{S} - \mathbf{A}^T\mathbf{R}_0))$, causing the loss function to become NaN, the gradient to become zero, and the optimization process to terminate. \jiangran{In contrast, the matrix Fisher distribution can be continuously optimized and theoretically approach the Dirac distribution infinitely.}

    Additionally, the optimization process of our rotation Laplace distribution is not smooth. As the predicted mode gets closer to the ground truth, the gradient becomes larger, leading to noticeable oscillations. These results highlight the limitation of our approach, indicating a risk of learning instability.

    % One alternative to avoid the problem is to increase the clipping parameter $\epsilon$. As shown in Fig \ref{fig:dirac}, when $\epsilon=1e-6$, the optimization process becomes stable. Larger $\epsilon$ will sacrifice the optimization accuracy a little bit yet can hardly be noticed (see Tab. \ref{tab:dirac}).
    % In downstream tasks, the influence of the choice of $\epsilon$ negligibly small compared to other factors.

    However, we notice that the oscillation is not observed in downstream learning tasks such as image-based rotation regression discussed in the manuscript, or in simpler $\SO$ learning tasks like Wahba's problem (as detailed in the next paragraph). 
    This absence of oscillation may be attributed to the difficulty of the predicted mode being accurate enough to trigger instability.
    % and the advanced optimizer (e.g., Adam with the gradient momentum).

    We include these analyses of singularities in Section 4.6 and Section 5.7 of our revised manuscript. 

    \begin{figure*}[th]
        \centering
        \begin{tabular}{ccc}
        \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_90_1.pdf} &
        \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_94_1.pdf} & 
        \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_95_1.pdf} \\
        \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_90_0.pdf} &
        \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_94_0.pdf} & 
        \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_95_0.pdf} \\
        % \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_90_2.pdf} &
        % \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_94_2.pdf} & 
        % \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_95_2.pdf} \\
        lr = 1e-4  & lr = 5e-4  & lr = 1e-3 \\        
        \end{tabular}
        \caption{\textbf{Visualization of the optimization curves of fitting a Dirac distribution.} We let the matrix Fisher distribution and rotation Laplace distribution to fit a Dirac distribution and plot the training curves. 
        % \jiangran{The optimization with matrix Fisher distribution does not converge in the figures.}
        }
        \label{fig:dirac}
    \end{figure*}

\end{itemize}


\textbf{Experiments on the Instance-level Wahba's problem: }
% The main advantage of rotation Laplace distribution is its robustness to the disturbance of outlier data points, for which our distribution achieves superior performance in many datasets. However, we do not claim a general dominance over other distributions. For example, in the category-level Wahba's problem experiments in the manuscript, our distribution achieves comparable performance as the competitors.
% To further examine the behavior of our distribution, we conduct a simpler experiment on the instance-level Wahba's problem.
\jiangran{To further investigate the behavior of our distribution in scenarios with few outliers and easy optimization, we conduct a simpler experiment on the instance-level Wahba's problem.}
Unlike the category-level setting in our previous manuscript, which is trained on thousands of airplane point clouds with random rotations (similar to \cite{zhou2019continuity, peretroukhin2020smooth}), this instance-level experiment focuses only on a single instance. Specifically, we choose an airplane point cloud from the ShapeNet dataset and apply random rotations in both the training and evaluation phases. The training process involves 10k iterations using the Adam optimizer, with a batch size of 100, and we experiment with different learning rates. The test errors throughout the learning process are depicted in Fig. \ref{fig:wahba_instance}. We set $\epsilon=1e-8$ for the rotation Laplace distribution.

For this simple task with perfectly annotated ground truth, our rotation Laplace distribution does not exhibit superiority. As shown in Fig. \ref{fig:wahba_instance}, our distribution achieves nearly identical performance to the matrix Fisher distribution and is slightly inferior to 10D \cite{peretroukhin2020smooth} in most cases. 
\jiangran{This simple Wahba's problem reveals that the rotation Laplace distribution is more suitable for scenarios with noticeable outliers.}

\jiangran{Furthermore, as mentioned in the previous paragraph, the rotation Laplace distribution does not suffer from oscillation in the learning process, which may be attributed to the difficulty of the predicted mode being accurate enough to trigger instability.}

We include experiments on Wahba's problem with instance-level settings in the supplementary.

\begin{figure*}[th]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.35\linewidth]{figures/response2/wahba_test_39.pdf} \hspace{2mm} &
    \includegraphics[width=0.35\linewidth]{figures/response2/wahba_test_40.pdf} 
    \vspace{-2mm}    \\ 
    lr=$1e-5$  \hspace{2mm} &  lr=$1e-4$ \\
    \includegraphics[width=0.35\linewidth]{figures/response2/wahba_test_41.pdf} \hspace{2mm} &
    \includegraphics[width=0.35\linewidth]{figures/response2/wahba_test_42.pdf} 
    \vspace{-2mm}    \\ 
    lr=$1e-3$  \hspace{2mm} &  lr=$1e-2$ \\     
    \end{tabular}
    \caption{\textbf{Visualization of the learning curves for instance-level Wahba's Problem.}}
    \label{fig:wahba_instance}
\end{figure*}

\textbf{In summary}, our proposed rotation Laplace distribution has two singularities: when $\mathbf{S}$ is close to zero and when the predicted mode is close to the ground truth. These singularities may lead to undesirable learning behaviors, presenting a fundamental limitation of our method. Specifically, our distribution is unable to fit a distribution with very large uncertainties, such as a uniform distribution, and it may suffer from unstable training when the predicted mode is very close to the ground truth. These phenomena may introduce potential issues in its usage. Designing a more elegant distribution that does not suffer from the aforementioned singularities is an important direction for future research. 

\jiangran{We also notice that rotation Laplace distribution does not consistently outperform other methods in all situations, as demonstrated in the instance-level Wahba's problem, which has minimal outliers during the learning process.} 
However, as demonstrated in many downstream experiments, the rotation Laplace distribution still exhibit a broad usability to a wide range of downstream applications, ranging from the simple instance-level Wahba's problem to the complex image-based rotation or 6D pose estimation. 

As the consistent stance of this article, we do not claim a general superiority of the rotation Laplace distribution over other representations in all scenarios, nor do we aim to replace existing methods.
However, with its strong robustness to the disturbance of outlier data points and the significant performance improvement in many real-world applications, we strongly believe that our proposed method offers a worthwhile alternative for users.
}


\begin{comment}


\setlength{\tabcolsep}{12pt}
\begin{table*}[th]
    \centering
    \small
    \caption{\textbf{Optimization results of fitting a Dirac distribution.} We let the matrix Fisher distribution and rotation Laplace distribution to fit a Dirac distribution and show the error after convergence. 
    % (Matrix Fisher distribution needs more iterations to converge than shown in Fig. \ref{fig:dirac}).
    }
    \begin{tabular}{cccc}
    \toprule
    & Matrix Fisher & \makecell{Rotation Laplace \\($\epsilon=1e-8$)}  &  \makecell{Rotation Laplace \\($\epsilon=1e-6$)} \\
    \midrule
    Error ($^\circ$)  &  0.406  & 0.405  & 0.408 \\
     \bottomrule
    \end{tabular}
    \label{tab:dirac}
\end{table*}

\begin{figure*}[th]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.35\linewidth]{figures/response2/wahba_test_90_1.pdf} \hspace{2mm} &
    \includegraphics[width=0.35\linewidth]{figures/response2/wahba_test_103_1.pdf} \\ 
    \includegraphics[width=0.35\linewidth]{figures/response2/wahba_test_90_0.pdf} \hspace{2mm} &
    \includegraphics[width=0.35\linewidth]{figures/response2/wahba_test_103_0.pdf} \\
    $\epsilon=1e-8$  & $\epsilon=1e-6$ \\        
    \end{tabular}
    \caption{\textbf{Visualization of the optimization curves of fitting a Dirac distribution.} We let the matrix Fisher distribution and rotation Laplace distribution to fit a Dirac distribution and plot the training curves. 
    % The optimization with matrix Fisher distribution does not converge in the figures.
    }
    \label{fig:dirac}
\end{figure*}



\begin{figure*}[th]
    \centering
    \begin{tabular}{cccc}
    \centering \rotatebox{90}{Gradient descent} & 
    \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_90_1.pdf} &
    \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_94_1.pdf} & 
    \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_95_1.pdf} \\
    \centering  \rotatebox{90}{Adam} & 
    \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_80_1.pdf} &
    \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_84_1.pdf} & 
    \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_85_1.pdf} \\
    % \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_80_2.pdf} &
    % \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_85_2.pdf} & 
    % \includegraphics[width=0.3\linewidth]{figures/response2/wahba_test_88_2.pdf} \\
    & lr = 1e-4  & lr = 5e-4  & lr = 1e-3 \\        
    \end{tabular}
    \caption{ }
    \label{fig:uniform_fit}
\end{figure*}
    




Thank you for your insightful suggestion. We acknowledge that a notable limitation of our proposed rotational Laplace distribution is the presence of singularity around the mode. We identify two primary causes of these singularities during the optimization process and delve into their respective impacts.
Firstly, singularities occur when the predicted mode closely aligns with the ground truth. In such cases, the gradient can become excessively large, impeding stable optimization. This issue may be especially prominent when attempting to fit a Dirac distribution. Secondly, singularities arise when uncertainties are substantial, causing the parameter $S$ to approach zero. This scenario prevents the distribution from fitting situations with high uncertainty, such as a uniform distribution.
To verify these hypotheses, we conduct separate experiments focusing on fitting these two distributions. Additionally, to further analyze the impact of singularities on downstream tasks, we supplement our study with more extensive evaluations on Wahba's problem, incorporating simpler instance-level point cloud inputs.

\paragraph{Experiments on Fitting Dirac Distribution on $\mathbf{\SO}$}

We conduct experiments to investigate the singularity issue by fitting a Dirac distribution on $\SO$. Specifically, we randomly select a rotation and optimized the distribution coefficient using the NLL loss. For comparison, we also use the matrix Fisher distribution as a reference.

As shown in Fig. \ref{fig
}, the gradient of the rotational Laplace distribution surges at the beginning and remains high, in contrast to the matrix Fisher distribution. This indicates that the learning rate is crucial for the optimization process, as depicted in Fig. \ref{fig
}. A larger learning rate results in severe oscillations during the fitting process, whereas a moderate learning rate maintains stability.

However, we do not observe this oscillatory behavior in downstream learning tasks, such as image-based rotation regression discussed in the manuscript, or in simpler $\SO$ learning tasks like Wahba's problem, as detailed in the next paragraph. This absence of oscillation may be attributed to the stochastic nature of learning, which prevents the predicted mode from being too close to the ground truth.
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/response2/tmp/dirac_gradient.jpeg}
    \caption{\small}
    \label{fig:dirac_grad}
\end{figure*}

\begin{figure*}[h]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.4\linewidth]{figures/response2/tmp/dirac_lr.jpeg} &
    \includegraphics[width=0.4\linewidth]{figures/response2/tmp/dirac_lr_m.jpeg}
    \end{tabular}
    \caption{\small}
    \label{fig:dirac_lr}
\end{figure*}

\paragraph{Experiments on Fitting Uniform Distribution on $\mathbf{\SO}$}

We conduct experiments to investigate the singularity with large uncertainty by fitting a uniform distribution on $\SO$. Specifically, we uniformly sample rotations and optimize the distribution coefficient using the NLL loss. As illustrated in Fig. \ref{fig:uniform_hist}, we visualize the statistical distribution through a histogram after coverage. 
In comparison to the matrix Fisher distribution, the rotational Laplace distribution exhibits a biased distribution across each PDF grid, indicating its inadequacy in representing a uniform distribution. This result demonstrates that the rotational Laplace distribution is unsuitable for data that closely follows a uniform distribution.

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/response2/tmp/uniform_histogram.jpeg}
    \caption{\small}
    \label{fig:uniform_hist}
\end{figure*}

\paragraph{More validation on Wahba's Problem benchmark.}
We examine the singularity issue within the context of Wahba's problem.
\begin{problem} \textbf{Wahba's Problem}

Given two sets of n points $\{ p_1, p_2, ..., p_n\}$ and $\{ p_1^*, p_2^*, ..., p_n^*\}$, where $n\ge 2$, find the rotation matrix $\mathbf{R}$ which brings the first set into the best least squares coincidence with the second. That is, find $\mathbf{R}$ which minimizes
\begin{equation}
    \sum_{i=1}^{n} \| p_i^* - \mathbf{R}p_i\|^2
\end{equation}
\end{problem}

In our previously submitted manuscript, our experiments focus on a category-level setting, following the methodology outlined in \cite{zhou2019continuity, peretroukhin2020smooth}. Due to the varying geometries, the optimization zone may be far from the singularity trigger.
To simplify the task and explore the effect further, we conducte additional experiments in a simpler instance-level manner. Specifically, we selected three airplane point clouds from the ShapeNet dataset \cite{shapenet2015} and train separate networks for each instance. Throughout both the training and evaluation phases, the point clouds underwent random rotations. The training process involved 10,000 iterations using the Adam optimizer, with a batch size of 100, and we experimented with different learning rates.

The training and test error progressions across iterations are visually depicted in Figure \ref{fig
}. We observe that the learning process remains stable rather than oscillating. Additionally, the rotation Laplace distribution achieve performance nearly identical to that of the matrix Fisher distribution, and slightly inferior to 10D \cite{peretroukhin2020smooth} in most cases.

In conclusion, the presence of singularities does indeed limit the applicability of the rotation Laplace distribution in certain scenarios. However, this limitation does not significantly impact downstream $\SO$ learning tasks, including simple instance-level Wahba's problem. Meanwhile, we also acknowledge that rotation Laplace distribution does not consistently outperform other methods in all situations, as demonstrated in this simpler Wahba's problem, which has minimal outliers during the learning process.
As the consistent stance of this article, our goal is not to replace the matrix Fisher distribution or other rotation representations but to offer a supplementary alternative for users. For learning tasks with a high presence of outlier data, such as image-based rotation regression on ModelNet or Pascal3D, we recommend starting with the rotation Laplace distribution as the initial approach.

\end{comment}

==> sections/proof_fisher_full.tex <==
\begin{proof}
% We consider the random variable $\mathbf{R}\sim \mathcal{MF}(\mathbf{A})$, where the proper SVD of matrix $\mathbf{A}$ is given as $\mathbf{A} = \mathbf{USV}^T$. Denote $\mathbf{R}_0$ as the mode of $\mathcal{MF}(\mathbf{A})$, i.e., $\mathbf{R}_0 = \mathbf{UV}^T$.
% We further define $\mathbf{\widetilde{R}}=\mathbf{R}_0^T\mathbf{R}$, thus when $\mathbf{R}$ is near mode $\mathbf{R}_0$, $\mathbf{\widetilde{R}}$ is near $\mathbf{I}$. 
Apply proper SVD to matrix $\mathbf{A}$ as $\mathbf{A} = \mathbf{USV}^T$.
For $\mathbf{R}\sim \mathcal{MF}(\mathbf{A})$, we have
\begin{equation}
\label{eq:prdr}
\scriptsize
\begin{aligned}
    p(\mathbf{R})d\mathbf{R} &\propto \exp\left(\tr{\mathbf{A}^T\mathbf{R}}\right)\mathrm{d}\mathbf{R}   
    % =\exp(\tr{\mathbf{VSU^T}\mathbf{\hat{\mathbf{R}}\widetilde{R}}})\mathrm{d}\mathbf{\widetilde{R}}
    = \exp\left(\tr{\mathbf{S}\mathbf{V}^T\mathbf{\widetilde{R}}\mathbf{V}}\right)\mathrm{d}\mathbf{\widetilde{R}}
\end{aligned}
\end{equation}
With $\boldsymbol{\phi}  = (\log{\mathbf{\widetilde{R}}})^\vee \in \mathbb{R}^3$,
$\mathbf{\widetilde{R}}$ can be parameterized as 
\begin{equation}
\scriptsize
    \mathbf{\widetilde{R}}(\boldsymbol{\phi} )= 
    \exp(\hat{\boldsymbol{\phi}}) = 
    \mathbf{I}+\frac{\sin\len {\boldsymbol{\phi}}  }{\len {\boldsymbol{\phi}}}\hat{\boldsymbol{\phi}}
    + \frac{1-\cos\len {\boldsymbol{\phi}}}{{\len {\boldsymbol{\phi}}}^2}{\hat{\boldsymbol{\phi}}}^2
\end{equation}
and the Haar measure is given by
\begin{equation}
\label{eq:d_rwave}
\scriptsize
    d\mathbf{\widetilde{R}} 
    = \frac{1- \cos \len {\boldsymbol{\phi}}}{{4\pi^2 \len {\boldsymbol{\phi}}}^2}d\boldsymbol{\phi}
    = \left(\frac{1}{8\pi^2}+O(\len {\boldsymbol{\phi}})^2\right)d\boldsymbol{\phi}.
\end{equation}
Also, $\mathbf{\widetilde{R}}$ expanded at $\boldsymbol{\phi}=\mathbf{0}$ is computed as
\begin{equation}
\scriptsize
    \mathbf{\widetilde{R}} = \mathbf{I}+\hat{\boldsymbol{\phi}}+\frac{1}{2}\hat{\boldsymbol{\phi}}^2+O({\len {\boldsymbol{\phi}} }^3)\\ 
\end{equation}
Given 
\begin{equation}
\label{eq:vtrv}
\scriptsize
\begin{aligned}
    \mathbf{V}^T\mathbf{\widetilde{R}}\mathbf{V} &= \mathbf{I} + \mathbf{V}^T\hat{\boldsymbol{\phi}}\mathbf{V} + \frac{1}{2}\mathbf{V}^T\hat{\boldsymbol{\phi}}^2\mathbf{V}+O(\len{\boldsymbol{\phi}}^3) 
    = \mathbf{I}+\widehat{\mathbf{V}^T\boldsymbol{\phi}}+\frac{1}{2}\widehat{\mathbf{V}^T\boldsymbol{\phi}}^2+O({\len {\boldsymbol{\phi}} }^3)\\
    &= \left[\begin{array}{ccc}
        1-\frac{1}{2}(\mu_2^2+\mu_3^2) & \frac{1}{2}{\mu_1}{\mu_2}-\mu_3 & \frac{1}{2}{\mu_1}{\mu_3}+\mu_2 \\
        \frac{1}{2}{\mu_1}{\mu_2}+\mu_3 & 1-\frac{1}{2}(\mu_3^2+\mu_1^2) & \frac{1}{2}{\mu_2}{\mu_3}-\mu_1 \\
        \frac{1}{2}{\mu_1}{\mu_3}-\mu_2 & \frac{1}{2}{\mu_2}{\mu_3}+\mu_1 & 1-\frac{1}{2}(\mu_1^2+\mu_2^2)
        \end{array}\right] + O({\len {\boldsymbol{\phi}}}^3),
\end{aligned}
\end{equation}
where $(\mu_1,\mu_2,\mu_3)^T = \mathbf{V}^T\boldsymbol{\phi}$, we have
\begin{equation}
\label{eq:tr}
\scriptsize
\begin{aligned}
    \tr{\mathbf{S}\mathbf{V}^T\mathbf{\widetilde{R}}\mathbf{V}} = 
    \tr{\mathbf{S}} + \sum_{(i,j,k)\in I}-\frac{1}{2}(s_j+s_k)\mu_i^2+O({\len {\boldsymbol{\phi}}}^3) 
    =\tr{\mathbf{S}} -\frac{1}{2}\boldsymbol{\phi}^T\mathbf{V}
    % \operatorname{diag}(s_2+s_3,s_3+s_1,s_1+s_2)
    \left[\begin{smallmatrix}
        s_2 + s_3 &  &  \\
        & s_1 + s_3 &  \\
        &  & s_1 + s_2
        \end{smallmatrix}\right]
    \mathbf{V}^T\boldsymbol{\phi}
\end{aligned}
\end{equation}
Considering Eq. \ref{eq:prdr}, \ref{eq:d_rwave} and \ref{eq:tr},
\begin{equation}
\scriptsize
\label{eq:gauss}
\begin{aligned}
    p(\mathbf{R})d\mathbf{R} &\propto \exp\left(\tr{\mathbf{A}^T\mathbf{R}}\right)\mathrm{d}\mathbf{R}  
    % = \left(\frac{1}{8\pi^2}+O({\len {\boldsymbol{\phi}}}^2)\right)\exp\left(\tr{\mathbf{S}}\right)\exp\left(\sum_{(i,j,k)\in I}-\frac{1}{2}(s_j+s_k)\mu_i^2+O({\len {\boldsymbol{\phi}}}^3)\right)\mathrm{d}\boldsymbol{\phi} \\
    % % &= (\frac{1}{8\pi^2}\exp(\tr{S})\exp(-\frac{1}{2}(\mathbf{V}^T\boldsymbol{\phi})^T\operatorname{diag}(s_2+s_3,s_3+s_1,s_1+s_2)(\mathbf{V}^T\boldsymbol{\phi}) + O({\len {\boldsymbol{\phi}}}^2))d\boldsymbol{\phi} \\
    % &= \frac{1}{8\pi^2}
    % \exp(\tr{S})
    % \exp\left(-\frac{1}{2}\boldsymbol{\phi}^T\mathbf{V}
    % % \operatorname{diag}(s_2+s_3,s_3+s_1,s_1+s_2)
    % \left[\begin{smallmatrix}
    %     s_2 + s_3 &  &  \\
    %     & s_1 + s_3 &  \\
    %     &  & s_1 + s_2
    %     \end{smallmatrix}\right]
    % \mathbf{V}^T\boldsymbol{\phi}\right)+ O({\len {\boldsymbol{\phi}}}^2)\mathrm{d}\boldsymbol{\phi} \\
    = \frac{\exp(\tr{S})}{8\pi^2}\exp\left(-\frac{1}{2}\boldsymbol{\phi}^T\boldsymbol{\Sigma} ^{-1}\boldsymbol{\phi}\right) \left(1 + O({\len {\boldsymbol{\phi}}}^2)\right)\mathrm{d}\boldsymbol{\phi}
\end{aligned}
\end{equation}
When $\mathbf{R}\rightarrow \mathbf{R}_0$, $\mathbf{\widetilde{R}} \rightarrow \mathbf{0}$ and $\boldsymbol{\phi} \rightarrow \mathbf{0}$, so Eq. \ref{eq:gauss} follows the multivariate Gaussian distribution 
with the covariance matrix as $\boldsymbol{\Sigma}$, where $\boldsymbol{\Sigma} = \mathbf{V}\operatorname{diag}(\frac{1}{s_2+s_3},\frac{1}{s_1+s_3},\frac{1}{s_1+s_2})\mathbf{V}^T$.
\end{proof}

==> sections/proof_laplace.tex <==
\begin{proof}

Apply proper SVD to matrix $\mathbf{A}$ as $\mathbf{A} = \mathbf{USV}^T$.
For $\mathbf{R}\sim \mathcal{RL}(\mathbf{A})$ , we have
\begin{equation}
\label{eq:prdr}
\scriptsize
\begin{aligned}
    p(\mathbf{R})\mathrm{d}\mathbf{R} &\propto 
    \frac{\exp\left(-\sqrt{\tr{\mathbf{S}-{\mathbf{A}^T\mathbf{R}}}}\right)}{\sqrt{\tr{\mathbf{S}-{\mathbf{A}^T\mathbf{R}}}}} \mathrm{d}\mathbf{R}
    = \frac{\exp\left(-\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{V}\mathbf{S}\mathbf{U}^T\mathbf{R})}\right)}{\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{V}\mathbf{S}\mathbf{U}^T\mathbf{R})}} \mathrm{d}\mathbf{R} \\
 &= \frac{\exp\left(-\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{U}^T\mathbf{R}\mathbf{V})}\right)}{\sqrt{\operatorname{tr}(\mathbf{S}-\mathbf{S}\mathbf{U}^T\mathbf{R}\mathbf{V})}} \mathrm{d}\mathbf{R} \\
    &= \frac{\exp\left(-\sqrt{\tr{\mathbf{S}-\mathbf{S}\mathbf{V}^T\mathbf{\widetilde{R}}\mathbf{V}}}\right)}{\sqrt{\tr{\mathbf{S}-\mathbf{S}\mathbf{V}^T\mathbf{\widetilde{R}}\mathbf{V}}}} \mathrm{d}\mathbf{R}
\end{aligned}
\end{equation}

% \jiangran{\input{sections_supp/elaboration.tex}}

With $\boldsymbol{\phi}  = (\log{\mathbf{\widetilde{R}}})^\vee \in \mathbb{R}^3$,
$\mathbf{\widetilde{R}}$ can be parameterized as 
{\footnotesize\begin{equation*}
    \mathbf{\widetilde{R}}(\boldsymbol{\phi} )= 
    \exp(\hat{\boldsymbol{\phi}}) = 
    \mathbf{I}+\frac{\sin\len {\boldsymbol{\phi}}  }{\len {\boldsymbol{\phi}}}\hat{\boldsymbol{\phi}}
    + \frac{1-\cos\len {\boldsymbol{\phi}}}{{\len {\boldsymbol{\phi}}}^2}{\hat{\boldsymbol{\phi}}}^2
\end{equation*}
}\ree{We follow the common practice \cite{mohlin2020probabilistic,lee2018bayesian} that the Haar measure $\mathrm{d}\mathbf{R}$ is scaled such that $\int_{SO(3)} \mathrm{d} \mathbf{R}=1$} and thus the Haar measure is given by
% and the Haar measure \ree{\cite{mohlin2020probabilistic,lee2018bayesian} is given by}
\begin{equation}
\footnotesize
\label{eq:d_rwave}
    \mathrm{d}\mathbf{\widetilde{R}} 
    = \frac{1- \cos \len {\boldsymbol{\phi}}}{{4\pi^2 \len {\boldsymbol{\phi}}}^2}\mathrm{d}\boldsymbol{\phi}
    = \left(\frac{1}{8\pi^2}+O(\len {\boldsymbol{\phi}})^2\right)\mathrm{d}\boldsymbol{\phi}.
\end{equation}
Also, $\mathbf{\widetilde{R}}$ expanded at $\boldsymbol{\phi}=\mathbf{0}$ is computed as 
{\small$\mathbf{\widetilde{R}} = \mathbf{I}+\hat{\boldsymbol{\phi}}+\frac{1}{2}\hat{\boldsymbol{\phi}}^2+O({\len {\boldsymbol{\phi}} }^3)$},
% {\scriptsize\begin{equation*}
%     \mathbf{\widetilde{R}} = \mathbf{I}+\hat{\boldsymbol{\phi}}+\frac{1}{2}\hat{\boldsymbol{\phi}}^2+O({\len {\boldsymbol{\phi}} }^3)\\ 
% \end{equation*}}
we have 
\begin{equation}
\label{eq:vtrv}
\scriptsize
\begin{aligned}
    \mathbf{V}^T\mathbf{\widetilde{R}}\mathbf{V} &= \mathbf{I} + \mathbf{V}^T\hat{\boldsymbol{\phi}}\mathbf{V} + \frac{1}{2}\mathbf{V}^T\hat{\boldsymbol{\phi}}^2\mathbf{V}+O(\len{\boldsymbol{\phi}}^3)\\
    &= \mathbf{I}+\widehat{\mathbf{V}^T\boldsymbol{\phi}}+\frac{1}{2}\widehat{\mathbf{V}^T\boldsymbol{\phi}}^2+O({\len {\boldsymbol{\phi}} }^3)\\
    &= \left[\begin{array}{ccc}
        1-\frac{1}{2}(\mu_2^2+\mu_3^2) & \frac{1}{2}{\mu_1}{\mu_2}-\mu_3 & \frac{1}{2}{\mu_1}{\mu_3}+\mu_2 \\
        \frac{1}{2}{\mu_1}{\mu_2}+\mu_3 & 1-\frac{1}{2}(\mu_3^2+\mu_1^2) & \frac{1}{2}{\mu_2}{\mu_3}-\mu_1 \\
        \frac{1}{2}{\mu_1}{\mu_3}-\mu_2 & \frac{1}{2}{\mu_2}{\mu_3}+\mu_1 & 1-\frac{1}{2}(\mu_1^2+\mu_2^2)
        \end{array}\right] \\ &+ O({\len {\boldsymbol{\phi}}}^3), 
\end{aligned}
\end{equation}
where $(\mu_1,\mu_2,\mu_3)^T = \mathbf{V}^T\boldsymbol{\phi}$, 
and
\begin{equation}
\label{eq:tr_laplace}
\footnotesize
\begin{aligned}
    \tr{\mathbf{S}-\mathbf{S}\mathbf{V}^T\mathbf{\widetilde{R}}\mathbf{V}} 
    &=\sum_{(i,j,k)\in I}\frac{1}{2}(s_j+s_k)\mu_i^2+O({\len {\boldsymbol{\phi}}}^3)\\ 
    % &=\frac{1}{2}(\mathbf{V}^T\phi)^T\operatorname{diag}(s_2+s_3,s_3+s_1,s_1+s_2)(\mathbf{V}^T\phi))+O({\len {\boldsymbol{\phi}}}^3) \\
    &=\frac{1}{2}\boldsymbol{\phi}^T\mathbf{V}
    % \operatorname{diag}(s_2+s_3,s_3+s_1,s_1+s_2)
    \left[\begin{smallmatrix}
        s_2 + s_3 &  &  \\
        & s_1 + s_3 &  \\
        &  & s_1 + s_2
        \end{smallmatrix}\right]
    \mathbf{V}^T\boldsymbol{\phi}+O({\len {\boldsymbol{\phi}}}^3)
\end{aligned}
\end{equation}
Considering Eq. \ref{eq:prdr}, \ref{eq:d_rwave} and \ref{eq:tr_laplace}, we have
\begin{equation}
\label{eq:laplace}
\footnotesize
\begin{aligned}
    p(\mathbf{R})\mathrm{d}\mathbf{R} &\propto \frac{\exp\left(-\sqrt{\tr{\mathbf{S}-{\mathbf{A}^T\mathbf{R}}}}\right)}{\sqrt{\tr{\mathbf{S}-{\mathbf{A}^T\mathbf{R}}}}} \mathrm{d}\mathbf{R}\\
    % = (\frac{1}{8\pi^2} + O({\len {\boldsymbol{\phi}}}^2))\frac{\exp(-\sqrt{\frac{1}{2}
    % \boldsymbol{\phi}^T\mathbf{V}
    % % \operatorname{diag}(s_2+s_3,s_3+s_1,s_1+s_2)
    % \left[\begin{smallmatrix}
    %     s_2 + s_3 &  &  \\
    %     & s_1 + s_3 &  \\
    %     &  & s_1 + s_2
    %     \end{smallmatrix}\right]
    % \mathbf{V}^T\boldsymbol{\phi}
    % +O({\len {\boldsymbol{\phi}}}^3)})}{\sqrt{\frac{1}{2}
    % \boldsymbol{\phi}^T\mathbf{V}
    % % \operatorname{diag}(s_2+s_3,s_3+s_1,s_1+s_2)
    % \left[\begin{smallmatrix}
    %     s_2 + s_3 &  &  \\
    %     & s_1 + s_3 &  \\
    %     &  & s_1 + s_2
    %     \end{smallmatrix}\right]
    % \mathbf{V}^T\boldsymbol{\phi}
    % +O({\len {\boldsymbol{\phi}}}^3)}}d\boldsymbol{\phi} \\
    &= \frac{1}{8\pi^2}\frac{\exp\left(-\sqrt{2\boldsymbol{\phi}^T\boldsymbol{\Sigma} ^{-1}\boldsymbol{\phi}}\right)}{\sqrt{2\boldsymbol{\phi}^T\boldsymbol{\Sigma} ^{-1}\boldsymbol{\phi}}}\left(1+ O({\len {\boldsymbol{\phi}}}^2)\right) \mathrm{d}\boldsymbol{\phi} \\
\end{aligned}
\end{equation}
When 
% $\mathbf{R}\rightarrow \mathbf{R}_0$
\ree{$\|\mathbf{R} - \mathbf{R}_0\| \rightarrow 0$}
, we have 
% $\mathbf{\widetilde{R}} \rightarrow \mathbf{I}$ 
\ree{$\|\mathbf{\widetilde{R}} - \mathbf{I}\|  \rightarrow 0$ }
and $\boldsymbol{\phi} \rightarrow \mathbf{0}$, so Eq. \ref{eq:laplace} follows the multivariate Laplace distribution 
with the covariance matrix as $\boldsymbol{\Sigma}$, where $\boldsymbol{\Sigma} = 4 \mathbf{V}\operatorname{diag}(\frac{1}{s_2+s_3},\frac{1}{s_1+s_3},\frac{1}{s_1+s_2})\mathbf{V}^T$.
\end{proof}

==> sections/tab_ablation.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[t]
    \caption{\small Numerical comparisons with our proposed Quaternion \& rotation Laplace distribution and baselines on ModelNet10-SO3 dataset. One model is trained for each category. Quaternion Laplace distribution clearly outperforms Bingham distribution \cite{deng2022deep}.}
    \vspace{2mm}
    \centering
    \scriptsize
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{}&& Chair &&&Sofa&&& Toilet&&&Bed&\\
    \cmidrule{2-13}  
        & Mean$\downarrow$ & Med.$\downarrow$ & Acc@5$\uparrow$ 
        & Mean$\downarrow$ & Med.$\downarrow$ & Acc@5$\uparrow$ 
        & Mean$\downarrow$ & Med.$\downarrow$ & Acc@5$\uparrow$ 
        & Mean$\downarrow$ & Med.$\downarrow$ & Acc@5$\uparrow$ 
        \\
        \midrule   
        Deng \textit{et al.}\cite{deng2022deep} & 16.5 & 7.2 & 0.31 & 16.5 & 4.9 & 0.52 & 9.6 & 4.2 & 0.59 & 22.0 & 5.1 & 0.49\\
        Mohlin \textit{et al.}\cite{mohlin2020probabilistic} & 10.8 & 4.6 & 0.55 & 11.1 & 3.5 & 0.70 & 6.4 & 3.5 & 0.70 & 16.0 & 3.8 & 0.66 \\
        \midrule
        % chair:543k, sofa:343.5k, toilet:597k, bed:573k
        quat. Laplace & 12.6 & 5.2 & 0.49 & 13.1 & 3.7 & 0.67 & 5.9 & 3.4 & 0.69 & 17.7 & 3.4 & 0.69\\
        rot. Laplace & \textbf{9.7}  & \textbf{3.5}  &  \textbf{0.68} & \textbf{8.8} & \textbf{2.1} & \textbf{0.84}  & \textbf{5.3} & \textbf{2.6} & \textbf{0.83} & \textbf{15.5} & \textbf{2.3} & \textbf{0.82}  \\
        % RLaplace-RPMG code base & {11.0}  & {4.0}  &  {0.61} & {10.0} & {2.3} & {0.82}  & {7.6} & {3.0} & {0.76} & {18.6} & {3.0} & {0.76}  \\
        \bottomrule
    \end{tabular}
  \label{tab:ablation}
\end{table*}



% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[t]
%   \centering
%   \fontsize{7.5}{9}\selectfont
%   \caption{Numerical comparisons with Quaternion Laplace distribution on ModelNet10-SO3 dataset. The results are averaged on all categories.}
%     \begin{tabular}{lcccccc}
%     \toprule
%           & Acc@3$^\circ$$\uparrow$ & Acc@5$^\circ$$\uparrow$ & Acc@10$^\circ$$\uparrow$ & Acc@15$^\circ$$\uparrow$ & Acc@30$^\circ$$\uparrow$ & Med.($^\circ$)$\downarrow$  \\
%     \midrule
    
%     \cite{deng2022deep}             &  (0.138)&   (0.301)&  (0.502)&  0.562 (0.584)&  0.694 (0.673)&   32.6 (31.6)\\
%     % modelnet/original_1, 43epoch
%     Mohlin \textit{et al.}\cite{mohlin2020probabilistic}  &  (0.164)& (0.389) &  (0.615) &  0.693 (0.684)&  0.757 (0.751)&   17.1 (17.9) \\
%     \midrule
%     rotation Laplace                 &       &       &       &       &       &        \\
%     Quaternion Laplace                    &       &       &       &       &       &        \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:ablation}%
% \end{table}%

